Event Detection from Social Media for Epidemic Prediction

Social media is an easy-to-access platform providing timely updates about societal trends and events. Discussions regarding epidemic-related events such as infections, symptoms, and social interactions can be crucial for informing policymaking during epidemic outbreaks. In our work, we pioneer exploiting Event Detection (ED) for better preparedness and early warnings of any upcoming epidemic by developing a framework to extract and analyze epidemic-related events from social media posts. To this end, we curate an epidemic event ontology comprising seven disease-agnostic event types and construct a Twitter dataset SPEED with human-annotated events focused on the COVID-19 pandemic. Experimentation reveals how ED models trained on COVID-based SPEED can effectively detect epidemic events for three unseen epidemics of Monkeypox, Zika, and Dengue; while models trained on existing ED datasets fail miserably. Furthermore, we show that reporting sharp increases in the extracted events by our framework can provide warnings 4-9 weeks earlier than the WHO epidemic declaration for Monkeypox. This utility of our framework lays the foundations for better preparedness against emerging epidemics.

==> sections/combined-benchmarking.tex <==
\section{Benchmarking ED Models}
\label{sec:combined-benchmarking}

We split and utilize our \dataName{} dataset (data splits in \S~\ref{sec:test-suites-statistics}) for benchmarking ED models.
Following \citet{ahn-2006-stages}, we report the F1-score for trigger identification (\textbf{Tri-I}) and classification (\textbf{Tri-C}).
% We majorly compare how utilizing limited \dataName{} data for training 
% Here, we present results for transferring existing ED models (without using any \dataName{} data) and training ED models with limited \dataName{} data.
Model and implementation details are provided in \S~\ref{sec:implementation-details}.

\input{sections/prev-work-results}

\input{sections/limited-data-results}



==> sections/data_analysis.tex <==
\section{Data Analysis}
\label{sec:data-analysis}
% \tanmay{Not complete/ready yet}

% \begin{table*}[ht]
%     \centering
%     \begin{tabular}{lrrrrrr}
%         \toprule
%         \multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Source}} & \textbf{Sentence} & \textbf{Event} & \textbf{Social} & \textbf{Personal} & \textbf{Medical} \\
%         & & \textbf{Granularity} & \textbf{Detection} & \textbf{Events} & \textbf{Events} & \textbf{Events} \\
%         \midrule
%         \dataName{} & Twitter & \cmark & \cmark & \cmark & \cmark &
%         \cmark \\
%         COVIDKB & Twitter & \cmark & \cmark & \xmark & \textbf{\texttildelow} & \textbf{\texttildelow} \\
%         BioCaster & News & \textbf{\texttildelow} & \textbf{\texttildelow} & \xmark & \xmark & \textbf{\texttildelow} \\
%         DANIEL &  & \xmark & \xmark & \xmark & \xmark & \xmark \\
%         Medical Reports & News & \cmark & \xmark & \xmark & \xmark & \xmark \\
%         PADI-Web & News \textbf{\texttildelow} & \xmark & \xmark & \xmark & \xmark \\
%         CACT & Clinical & \\
%         \bottomrule
%     \end{tabular}
%     \caption{Data Statistics for \dataName{} FILL, I ADDED PIFONT IN MAIN AND XMARK CMARK IN MACROS}
%     \label{tab:data-statistics}
% \end{table*}

% Our dataset \dataName{} comprises seven event types with $2$,$217$ event mentions annotated over $1$,$975$ tweets.
% In this section, we provide an objective comparison of our dataset with other epidemiological datasets (\S~\ref{sec:dataset-comparison}) along with some quantitative analyses for comparison with standard ED datasets (\S~\ref{sec:quantitative-analysis}).
% Detailed statistics are presented in the Appendix \ref{sec:data-analysis-appendix}.

In this section we present quantitative analyses of our dataset for comparison with other standard ED datasets.
Comparison with other epidemiological datasets is discussed in \S~\ref{sec:related-works} along with an objective comparison in Table~\ref{tab:dataset-checklist}.

% \subsection{Epidemiological Datasets Comparison}
% \label{sec:dataset-comparison}

% We provide an objective comparison of our \dataName{} dataset relative to other related epidemiological datasets in Table~\ref{tab:dataset-checklist}.
% % \tanmay{Maybe include trigger annotation column}
% We show how most datasets focus on clinical/news sources, are not annotated at the sentence level\footnote {We treat each tweet as a sentence for comparison.} granularity, and do not possess trigger information for ED.
% ExcavatorCovid \cite{min-etal-2021-excavatorcovid} and BioCaster \cite{DBLP:journals/bioinformatics/CollierDKGCTNDKTST08} provide great event coverage but are too fine-grained for social media.
% COVIDKB \cite{zong-etal-2022-extracting} uses Twitter, but it covers a smaller range of event types and focuses on the slot-filling task.
% % \wei{we may want to furnish comparison of these 3 covid related datasets in Table 3}
% \dataName{} is the only dataset that is well-annotated for sentence-level ED, granular for social media events, and possesses a decent event coverage.
% \tanmay{How should we handle this section? Should we keep this + table here / appendix?}
% \kuanhao{Discuss in related work + appendix. Shift table too.}
% \tanmay{Can remove this section / discuss in related works. Can move table to Appendix. Majorly, we observe that the reviewers we get are not epidemiological folks, so it's not adding high value.}

% \kuanhao{can be moved to appendix}
% We provide the major statistics for \dataName{} and compare it with other standard ED datasets like ACE \cite{doddington-etal-2004-automatic}, ERE \cite{song-etal-2015-light}, and MAVEN \cite{wang-etal-2020-maven} in Table~\ref{tab:data-statistics}.
% % \tanmay{@Bonnie, I've created the table barebone. Please add numbers to it}
% We have a relatively smaller dataset in terms of sentences and event mentions as we focus only on epidemic events.
% But our dataset is decently dense as it has a par average number of event mentions per event.
% Another strong distinction relative to other datasets is that our data source is Twitter while it's news for ACE/ERE and Wikipedia for MAVEN.
% Avg. sentences/mentions per Event is at par with other datasets.
% Show the difference by some metric b/w news/wiki/twitter datasets and the challenges associated.

% \tanmay{@Kuan-Hao, should we also compare with epidemiological datasets? It's not doable directly, but is it worth?}

% \begin{enumerate}
    % \item Add main table with basic statistics about our dataset and compare with existing ED datasets \tanmay{@Bonnie}
    % \item Discuss the difference in mean or distribution of length of sentences / event density (token-level) / perplexity (if exists) \tanmay{@Bonnie}
% \end{enumerate}

% \subsection{Quantitative Analysis}
% \label{sec:quantitative-analysis}
% \tanmay{@Bonnie}

\paragraph{Data Statistics}
Our dataset \dataName{} comprises seven event types with $2$,$217$ event mentions annotated over $1$,$975$ tweets.
% Apart from basic statistics, we provide some quantitative analysis of our dataset in this section.
We compare \dataName{} with other standard ED datasets like ACE \cite{doddington-etal-2004-automatic}, ERE \cite{song-etal-2015-light}, and MAVEN \cite{wang-etal-2020-maven} in Table~\ref{tab:data-statistics}.
% \kuanhao{Add column for data source}
% \kuanhao{Can add other dataset from OmniEvent paper}
Despite the lesser number of sentences and event mentions (since we focus only on $7$ event types),
\dataName{} has a reasonable size of $316$ average event mentions per event, which is more than the standard ACE and ERE datasets.
We also note the differences of the domain of data sources as ACE/ERE focus on News, MAVEN on Wikipedia, while \dataName{} is based on social media, specifically Twitter data.

\begin{table}[t]
    \centering
    \small
    \setlength{\tabcolsep}{.9pt}
    \begin{tabular}{lccccc}
        \toprule
        % \mu ltirow{2}{*}{\textbf{\# ET}}
        % \multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{\# Sentences}} & \multirow{2}{*}{\textbf{\# Tokens}} & \textbf{\# Event} & \textbf{\# Event} & \textbf{Avg. Mentions} \\
        % & & & \textbf{Types} & \textbf{Mentions} & \textbf{per Event} \\
        \multirow{2}{*}{\textbf{Dataset}} & \textbf{\# Event} & \multirow{2}{*}{\textbf{\# Sent}} & \multirow{2}{*}{\textbf{\# EM}} & \textbf{Avg. EM} & \multirow{2}{*}{\textbf{Domain}} \\
        & \textbf{Types} & & & \textbf{per Event} \\
        \midrule
        \textbf{ACE} & $33$ & $18,927$ & $5,055$ & $153.2$ & News \\
        \textbf{ERE} & $38$ & $17,108$ & $7,284$ & $191.7$ & News \\
        \textbf{MAVEN} & $168$ & $49,873$ & $118,732$ & $706.$7 & Wikipedia \\
        % \midrule
        % \textbf{COVIDKB} & 5 & 10,000 & 5,177 & 1035.4 \\
        %\multirow{2}{*}{\textbf{\dataName}} & \multirow{2}{*}{$7$} & \multirow{2}{*}{$1,975$} & \multirow{2}{*}{$2,217$} & \multirow{2}{*}{$316.7$} & Social \\ & & & & & Media \\
        \textbf{\dataName} & $7$ & $1,975$ & $2,217$ & $316.7$ & Social Media \\
        \bottomrule
    \end{tabular}
    \caption{Data Statistics for \dataName{} dataset and comparison with other standard ED datasets. \# = ``number of", Avg. = average, Sent = sentences, EM = event mentions.}
    \label{tab:data-statistics}
\end{table}

% \paragraph{Event Type Distribution}
% As part of data processing, we attempt to sample tweets in a more uniform distribution between the event types (\S~\ref{sec:twitter-selection}).
% In Figure~\ref{fig:event-type-distribution}, we show the distribution of our dataset in terms of event types.
% In contrast to tail-ending distributions of other standard datasets (\S~\ref{sec:event-distribution-appendix}), our distribution of event mentions is more uniform.
% The utility of this uniform distribution for robust training and evaluation are discussed in \S~\ref{sec:event-based-sampling} and 
% \tanmay{@Alex add your section number here}.
% Say how it's better compared to tail-based distributions of other datasets and provides better uniform evaluation.
% \tanmay{@Bonnie add the pie-chart instead of the table here}
% \tanmay{Show comparison with random sampling to emphasize our sampling more}
% Add line about how our sampling method works and ensures uniform sampling which further helps with better model training and testing.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\columnwidth]{images/event_distribution.pdf}
%     \caption{Distribution of event mentions per event type for our dataset \dataName.}
%     \label{fig:event-type-distribution}
% \end{figure}

% \tanmay{If space, then add analysis for number of trigger words}

% \paragraph{Trigger Distribution}
% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=\columnwidth]{images/trigger_words.pdf}
%     \caption{Unique trigger words per event}
%     \label{fig:trigger-distribution}
% \end{figure}
% % \tanmay{@Bonnie add figure about distinct number of triggers}
% Add comparison with average number of distinct triggers with other datasets for an interesting distinction.

% \paragraph{Event Mention Density}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\columnwidth]{images/event_mentions.pdf}
%     \caption{Distribution of number event mentions per sentence. Here \% indicates percentage.}
%     \label{fig:event-mention-distribution}
% \end{figure}

% We compare the distribution of event mentions per sentence with other ED datasets like ACE \cite{doddington-etal-2004-automatic} and MAVEN \cite{wang-etal-2020-maven} in Figure~\ref{fig:event-mention-distribution}.
% We observe that the event density of our dataset is less than MAVEN but better than ACE.
% This shows that despite having just seven event types, \dataName{} is a fairly dense dataset.
% The distributions aren't comparable directly as previous datasets were annotated at the document level and comprise different event types.
% Some line about how our dataset is still relatively dense and we support multiple events per sentence.

% \tanmay{@Bonnie add figure for distribution of event mentions}
% Compare with other datasets and show the distribution is similar.

% \begin{enumerate}
%     \item Re-iterate the use of event-based sampling to ensure more uniform sampling. Can have a small study of event distribution if sampling was done uniformly. 
    
% \begin{table}[htbp]
%     \centering
%     \caption{Number of Occurrences Per Event}
%     \label{tab:results}
%     \begin{tabular}{|c|c|c|}
%         \hline
%         \textbf{Event} & \textbf{Number of Occurrences} \\
%         \hline
%         Control & 478 \\
%         Cure & 272 \\
%         Death & 519 \\
%         Infect & 342 \\
%         Prevent & 241 \\
%         Spread & 331 \\
%         Symptom & 216 \\
%         \hline
%     \end{tabular}
% \end{table}
% \end{enumerate}

\paragraph{Event Mention Density Analysis}
We compare the distribution of event mentions per sentence with other ED datasets like ACE and MAVEN in Figure~\ref{fig:event-mention-distribution}.
We observe that the event density of our dataset is less than MAVEN but better than ACE.
This shows that despite having just seven event types, \dataName{} is a fairly dense dataset.

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{images/event_mentions.pdf}
    \caption{Distribution of number event mentions per sentence. Here \% indicates percentage.}
    \label{fig:event-mention-distribution}
\end{figure}

\paragraph{Trigger Word Analysis}
\label{sec:trigger-word-analysis}

We show the diversity of trigger words in \dataName{} and compare it with other datasets in Table~\ref{tab:trigger-word-diversity}.
We note that \dataName{} has a strong average number of triggers per event mention.
This demonstrates how \dataName{} is a diverse and challenging ED dataset.

\begin{table}[t]
    \centering
    \small
    \begin{tabular}{lrr}
        \toprule
        \multirow{2}{*}{\textbf{Dataset}} & \textbf{\# Unique} & \textbf{Avg. Triggers} \\
        & \textbf{Triggers} & \textbf{per Mention} \\
        \midrule
        ACE & $1,229$ & $0.24$ \\
        MAVEN & $7,074$ & $0.06$ \\
        \dataName{} & $555$ & $\textbf{0.25}$ \\
        \bottomrule
    \end{tabular}
    \caption{Comparison of \dataName{} with ACE and MAVEN in terms of unique trigger words and average number of triggers per event mention. Avg = Average.}
    \label{tab:trigger-word-diversity}
\end{table}

% \subsection{Qualitative Analysis}
% % \tanmay{@Eric}

% % \begin{enumerate}
% %     \item Show some quality examples for a few events. Describe the tough cases of infect/spread or prevent/control here.
% %     \tanmay{@Eric}
% % \end{enumerate}

% \begin{table*}[ht]
%     \centering
%     \begin{tabular}{p{10.5cm}ll}
%         \toprule
%         \textbf{Event Mention} & \textbf{Event Type} & \textbf{Event Trigger} \\
%         \midrule
%         \multirow{2}{10.5cm}{My nephew in Minnesota has tested \textbf{positive} for COVID - he \textbf{has} a terrible headache and fever ...} & infect & positive \\
%         & symptom & has \\ \hline
%         With \textbf{spike} of close to 4000 cases, India's COVID-19 count reaches 85,940 on Saturday ... & spread & spike \\ \hline
%         ... It's not hard to wear a mask. Youre \textbf{protecting} yourself and others. & prevent & protecting \\ \hline
%         Keep 6 feet apart. Its on all of us to \textbf{prevent} the spread of \#COVID ... & control & prevent \\
%         \bottomrule
%     \end{tabular}
%     \caption{Qualitative examples of event mentions from our \dataName{} dataset.}
%     \label{tab:data-examples}
% \end{table*}

% We show examples of event mentions for several event types from our dataset in Table~\ref{tab:data-examples}.




==> sections/data_collection.tex <==
\section{Ontology Creation and Data Collection}
% \kuanhao{Change the section title to ontology construction and data collection?}
We choose social media as our document source since it provides faster and more timely worldly information than other alternatives like news and public health \cite{lamb-etal-2013-separating} and is more publicly accessible than clinical notes \cite{DBLP:journals/jbi/LybargerOTY21}.
Owing to its public access and huge content volume, we consider \textbf{Twitter}\footnote{\url{https://www.twitter.com/}} as the social media platform and consider the recent \textbf{COVID-19 pandemic} as the primary disease for our dataset.

Previous epidemiological ontologies are typically specific to a particular disease, too fine-grained, or cover only a few event types (\S~\ref{sec:epi-ontologies} and Table~\ref{tab:dataset-checklist}) and cannot be readily utilized for ED from social media.
Similarly, standard ED datasets don't comprise epidemiological events and are mostly confined to news or wikipedia domains (\S~\ref{sec:ed-datasets}).
Owing to these reasons, we create our own event ontology and dataset \dataName{} specific to detecting epidemics from social media.
We provide a brief overview of our data creation process in Figure~\ref{fig:dataset-creation-process} and discuss these steps in more detail below.
% \tanmay{Need to make change to ontology creation figure}

% In this section, we describe the process of creating our event ontology and dataset (Figure~\ref{fig:dataset-creation-process}).
% In \S~\ref{sec:ontology-creation}, we define our event ontology comprising epidemic preparedness events.
% We describe our data preprocessing in \S~\ref{sec:twitter-selection}.
% Finally, details about data annotation are provided in \S~\ref{sec:data-annotation}.
% We provide an illustration of our pipeline in Figure~\ref{fig:dataset-creation-process}.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\columnwidth]{images/dataset-creation-process.pdf}
    \caption{Overview of our dataset creation process.}
    \label{fig:dataset-creation-process}
\end{figure}
% \alex{Can move this eye-catching and informative illustration forward (Figure 3). The frist two pages are text-heavy }

% \begin{table*}[ht]
%     \centering
%     \begin{tabular}{l|p{10cm}|l}
%     \toprule
%     \textbf{Event Type} & \textbf{Definitions and Examples} & \textbf{Event Trigger} \\
%     \midrule
%     \multirow{ 2}{*}{Infect}
%     & The process of a disease/pathogen invading host(s).& catch \\& Eg. Children can \textbf{catch} COVID-19.\\
%     \midrule
%     \multirow{ 2}{*}{Spread}
%     & The process of a disease spreading/prevailing massively at a large scale. & RISE \\& Eg. COVID 19 CASES \textbf{RISE} TO 85,940  IN INDIA. (url)\\
%     \midrule
%     \multirow{ 2}{*}{Symptom}
%     & Individuals displaying physiological features indicating the abnormality of organisms. & coughing \\& Eg. (user) Still \textbf{coughing} two months later..\\
%     \midrule
%     \multirow{ 2}{*}{Prevent}
%     & Individuals trying to prevent the infection of a disease. & prevent \\& Eg. ...wearing face mask is a scientific measure to \textbf{prevent} COVID-19\\
%     \midrule
%     \multirow{ 2}{*}{Control}
%     & Collective efforts trying to impede the spread of a pandemic. & reduce \\& Eg. Social Distancing is the responsibility of all of us to \textbf{reduce} the spread of COVID-19...\\
%     \midrule
%     \multirow{ 2}{*}{Cure}
%     & Stopping infection and relieving individuals from infections/symptoms. & recovered \\ & Eg. ...\textbf{recovered} COVID-19 patients cant get it again.\\
%     \midrule
%     \multirow{ 2}{*}{Death}
%     & End of life of individuals due to infectious disease. & died \\& Eg. More than 80,000 Americans have \textbf{died} of coronavirus.\\

%     \bottomrule
%     \end{tabular}
%     \caption{Event ontology focused on events for predicting the next pandemic along with their definitions.}
%     \label{tab:event-ontology}
% \end{table*}

\subsection{Ontology Creation}
\label{sec:ontology-creation}

% To create an event ontology for predicting the next pandemic, we revisited some past epidemiological ontologies and later curated our event ontology.

% \mypar{Previous Epidemiological Ontologies}
% Majorly, we study four ontologies:
% (1) \textit{Human Disease Ontology} \cite{DBLP:journals/nar/SchrimlMSOMFBJB22} is a comprehensive knowledge ontology of human diseases categorized based on clinical, genetic, and biological characteristics.
% (2) \textit{Infectious Disease Ontology} \cite{DBLP:journals/biomedsem/BabcockBCS21} focuses on infectious human diseases along with germane pathogen entities and relationships.
% (3) \textit{Ontology of Coronavirus Infectious Disease} \cite{DBLP:conf/icbo/He0OWLHHBLDAXHY20} specializes in the coronavirus disease and corresponding etiology, transmission, pathogenesis, diagnosis, prevention, and treatment.
% (4) \textit{BioCaster Event Ontology} \cite{DBLP:journals/bioinformatics/CollierDKGCTNDKTST08} is a multilingual information network; less biomedically technical and targets more high-level events regarding pandemics.
% Most of these ontologies comprise extensive biomedical information and thus, are not directly suitable for social media text.
% The BioCaster ontology is much better suited, but its complete taxonomy still appears excessively detailed when applied to social media contents. Also, since the BioCaster disease surveillance system targets online news articles, a direct application of BCEO on Twitter text is subjected to a domain shift as information from social media is less synthesized.

% \looseness=-1
% Previous epidemiological ontologies are typically specific to a particular disease, too fine-grained, or cover only a few event types (\S~\ref{sec:epi-ontologies} and Table~\ref{tab:dataset-checklist}) and cannot be readily utilized for ED from social media.
% Taking inspiration from BCEO \cite{DBLP:journals/bioinformatics/CollierDKGCTNDKTST08}, IDO \cite{DBLP:journals/biomedsem/BabcockBCS21}, and the ExcavatorCovid \cite{DBLP:conf/emnlp/MinRQZXM21} ontologies, we create our ontology with a wide coverage of epidemic events that characterize any disease.
% % Inspired by these ontologies, we curate our event ontology with a focus on event types related to the inception, symptoms, spread, control policies, and mortality in a pandemic.
% Our initial ontology comprises $18$ event types organized into three abstractions of social (events involving larger populations), personal (individual-oriented events), and medical (medically focused events) types as reported in Table~\ref{tab:complete-ontology} (\S~\ref{sec:complete-ontology}).
% Based on our analysis of the relevance and frequency of these events in social media (\S~\ref{sec:initial-event-analysis}), we merge and discard some event types to create our final ontology of seven major event types that are better suited for social media.
% % Our final ontology comprises seven event types 
% % \wei{would the performance of the ED models be different if we use the original 18 event types?} \tanmay{We don't know. But annotation is simpler with 7 event types. That's the main reason.}
% % These events have better pairwise distinction and majorly originate from the social and personal domains as they are discussed more on social media.
% Finally, we validate our ontology and event definitions by a public health expert.
% Table~\ref{tab:event-ontology} enlists our final ontology with the event definitions and example event mentions.
% \tanmay{@Jiarui, add the definitions of these events. Also add one example sentence, ideally from our dataset. The sentence should be handpicked good and short if possible.}

% Previous epidemiological ontologies are typically specific to a particular disease, too fine-grained, or cover only a few event types (\S~\ref{sec:epi-ontologies} and Table~\ref{tab:dataset-checklist}) and cannot be readily utilized for ED from social media.
% To circumvent this issues of previous epidemiological ontologies, we create our ontology with a wide coverage of epidemic events that characterize any disease while taking inspiration from medical sources like BCEO \cite{DBLP:journals/bioinformatics/CollierDKGCTNDKTST08}, IDO \cite{DBLP:journals/biomedsem/BabcockBCS21}, and the ExcavatorCovid \cite{DBLP:conf/emnlp/MinRQZXM21} ontologies.
% , we create our ontology with a wide coverage of epidemic events that characterize any disease.
Taking inspiration from medical sources like BCEO \cite{DBLP:journals/bioinformatics/CollierDKGCTNDKTST08}, IDO \cite{DBLP:journals/biomedsem/BabcockBCS21}, and the ExcavatorCovid \cite{DBLP:conf/emnlp/MinRQZXM21}, we curate a wide range of epidemic events while ensuring that they are not biased for specific diseases.
We categorize these events into three abstractions of social (events involving larger populations), personal (individual-oriented events), and medical (medically focused events) types and create our initial ontology comprising $18$ event types as reported in Table~\ref{tab:complete-ontology} (\S~\ref{sec:complete-ontology}).
% Our initial ontology comprises $18$ event types organized into three abstractions of social (events involving larger populations), personal (individual-oriented events), and medical (medically focused events) types as reported in Table~\ref{tab:complete-ontology} (\S~\ref{sec:complete-ontology}).

\mypar{Social Media Relevance}
To adapt our curated ontology better for social media, we conduct a deeper analysis of the event types based on their frequency and relevance.
Majorly, we associate each event type with a certain set of keywords and rank them based on the confidence and frequency of the occurrence of their keywords in social media posts (more details in \S~\ref{sec:initial-event-analysis}).
Based on this relevance-based ranking, we merge and discard some event types.
Furthermore, we conduct human studies and merge event types to ensure better pairwise distinction.
% Based on our analysis of the relevance and frequency of these events in social media , we merge and discard some event types to create our final ontology of seven major event types that are better suited for social media.
% These events have better pairwise distinction and majorly originate from the social and personal domains as they are discussed more on social media.

\mypar{Ontology Validation and Coverage}
Drawing upon established epidemiological ontologies serves to guarantee the medical soundness of our ontology.
In addition, we assess the sufficiency and comprehensiveness of our ontology and definitions through evaluation by two public health experts.
% Derivation from existing epidemiological ontologies ensures the medical soundness of our ontology. 
% Furthermore, we validate the sufficiency and coverage of our ontology and event definitions by two public health experts.
We also quantify our ontology coverage for four diverse diseases by evaluating the percentage of event occurrence in disease-related tweets.
We observe a high coverage of $50\%$ for COVID-19, $44\%$ for Monkeypox, $70\%$ for Dengue and $73\%$ for Zika (more details in \S~\ref{sec:disease-coverage}), ensuring strong disease coverage of our ontology.
% \tanmay{Experiment to verify coverage of ontology}

Our final \dataName{} ontology comprises seven major event types that are better suited for social media and cover important aspects of an epidemic.
We present our ontology in Table~\ref{tab:event-ontology} along with event definitions and example event mentions.

% \mypar{Event ontology curation}
% Inspired by these ontologies, we curate our event ontology with a focus on event types related to the inception, symptoms, spread, control policies, and mortality in a pandemic.
% We create a large ontology of $7$ \tanmay{@Jiarui, fill the number here} events organized into three abstractions of social (pandemic events related to larger population), personal (individual-oriented pandemic events), and medical (medically focused pandemic events) domains.
% \tanmay{@Jiarui, add the whole ontology in a table in the Appendix organized by these three abstractions}
% Based on an initial analysis of the occurrence of these events in social media, we trim our event ontology into seven major events.
% These events have better pairwise distinction and majorly originate from the social and personal domains.
% We enlist our final ontology along with their definitions in Table~\ref{tab:event-ontology}.
% \tanmay{@Jiarui, add the definitions of these events. Also add one example sentence, ideally from our dataset. The sentence should be handpicked good and short if possible.}

% \begin{enumerate}
%     \item Discuss the previous ontologies from which we took inspiration for creating our ontology

% We created our ontology based on four extant infectious-diseases-related ontologies: the BioCaster Event Ontology (BCEO), Ontology of Coronavirus Infectious Disease (CIDO), Human Disease Ontology (DO), and Infectious Disease Ontology (IDO). 

% (1) DO \cite{DBLP:journals/nar/SchrimlMSOMFBJB22} is a standard ontology and provides comprehensive knowledge of a wide range of human diseases, which are categorized based on detailed clinical, genetic, and biological characteristics and listed hierarchically.

% (2) IDO \cite{DBLP:journals/biomedsem/BabcockBCS21} is also a popular knowledge structure, but with a specification in the domain of infectious human diseases compared to DO. Besides the standard categorization of each infectious disease, IDO also covers germane pathogen entities and relationships.

% (3) CIDO \cite{DBLP:conf/icbo/He0OWLHHBLDAXHY20} has a further specialized focus on the coronavirus infectious disease. By providing the etiology, transmission, pathogenesis, diagnosis, prevention, and treatment of each member of the coronavirus family, CIDO provides a comprehensive knowledge framework which facilitates computers’ interpretation of coronavirus diseases. 

% (4) As a component of the BioCaster disease surveillance system \cite{DBLP:journals/bioinformatics/CollierDKGCTNDKTST08}, BCEO is designed to presents a bridge between health experts’ knowledge and online disease reports as well as a multilingual information network. Differed from the above three ontologies, BCEO contains less detailed biomedical entities but includes more high-level relations and events regarding pandemic, each presented with multilingual synonym sets.

% Taking the union of the information from these four ontologies, we conclude that our pandemic related events can be categorized into three groups, depending on whether it is related to a social aspect (such as pandemic outbreak or control), personal aspect (such as infection or prevention), or a medical aspect (such as virus variant or transmission route). Two issues would occur if we kept the whole ontology: 1) the tweeter data contains very little mentions of medical events. 2) subtle nuance between events lead to discrepancies among annotators. Thus, we finalize our ontology with only seven events, which have relatively less pair-wise similarity and originate from social and personal aspects.
    
    % \item Create table of events and corresponding definitions here
    
% \end{enumerate}

\begin{table*}[ht]
    \centering
    \small
    \resizebox{.99\textwidth}{!}{
    \begin{tabular}{l|p{6.6cm}|p{6.6cm}}
    \toprule
    \textbf{Event Type} & \textbf{Event Definition} & \textbf{Example Event Mention} \\
    \midrule
    Infect & The process of a disease/pathogen invading host(s) & Children can also \textbf{catch} COVID-19 ... \\ \midrule
    Spread & The process of a disease spreading/prevailing massively at a large scale & \#COVID-19 CASES \textbf{RISE} TO 85,940  IN INDIA ... \\ \midrule
    Symptom & Individuals displaying physiological features indicating the abnormality of organisms & (user) (user) Still \textbf{coughing} two months after being infected by this stupid virus ... \\ \midrule
    Prevent & Individuals trying to prevent the infection of a disease & ... wearing mask is the way to \textbf{prevent} COVID-19 \\ \midrule
    Control & Collective efforts trying to impede the spread of epidemic & Social Distancing is our responsibility to \textbf{reduce} spread of COVID-19 ... \\ \midrule
    Cure & Stopping infection and relieving individuals from infections/symptoms & ... \textbf{recovered} corona virus patients cant get it again \\ \midrule
    Death & End of life of individuals due to infectious disease. & More than 80,000 Americans have \textbf{died} of COVID ... \\
    \bottomrule
    \end{tabular}}
    \caption{Event ontology comprising seven event types promoting epidemic preparedness along with their definitions and example event mentions. The trigger words are marked in \textbf{bold}.}
    \label{tab:event-ontology}
\end{table*}

\subsection{Data Processing}
\label{sec:twitter-selection}

% We require a large number of relevant documents to support annotation using our curated event ontology.
% We choose social media as the primary source of documents as it is an easily accessible source capturing the public sentiments of billions all over the world.
% We choose social media as our document source since it provides faster and more timely information than other alternatives like news and public health \cite{lamb-etal-2013-separating} and is more publicly accessible than clinical notes \cite{DBLP:journals/jbi/LybargerOTY21}.
% Compared to news, blogs, Wikipedia, and other domains, social media is more ubiquitously used by people all over the world and better captures the public sentiment.
% Thus, capturing large-scale information about epidemic events would be faster on social media than other standard sources \cite{lamb-etal-2013-separating}.
% Owing to its public access and huge content volume, we consider \textbf{Twitter}\footnote{\url{https://www.twitter.com/}} as the social media platform and consider the recent \textbf{COVID-19 pandemic} as the primary disease for our dataset.
% Despite these restrictions, we believe that our work and models can be easily extended to other social media platforms and for other pandemics too (as shown in \S~\ref{}\tanmay{Add reference}).

% \mypar{Data Source and Preprocessing}
To access a wide range of tweets related to COVID-19, we utilized the Twitter COVID-19 Endpoint released in April 2020.
% This endpoint helped filter out public tweets that are specifically related to COVID-19.
We used a randomized selection of \textbf{331 million tweets} between May 15 -- May 31 2020, as our base dataset.
% \mypar{Tweet Preprocessing}
For preprocessing tweets, we follow \citet{POTA2021115119}: (1) we anonymize personal information like phone numbers, emails, and handles, (2) we normalize any retweets and URLs, (3) we remove emojis and split hashtags, (4) we filter out tweets only in English.
% \alex{@Tanmay, please review once more} 

% Most of the tweets provided subjective opinions and public sentiment, which are not related to the events in our ontology.
% Our initial study revealed a HIT rate of merely 3\%, i.e. only 3\% of the tweets consist of event-related information.
% Annotating a random sample of these tweets would be resource-expensive and yield very few datapoints for event extraction.
% Thus, we focus our efforts on filtering these tweets to improve the HIT rate.

\mypar{Event-based Filtering}
Despite COVID-based filtering, most tweets in our base dataset expressed subjective public sentiments, while only 3\% comprised mentions adhering to our curated event ontology.\footnote{Based on keyword-based study conducted on 1,000 tweets}
To reduce annotation costs, we further filter these tweets based on our curated ontology using a simple \textit{sentence embedding} similarity technique.
% The goal of this filtering step is to select tweets suspected to be more related to our event ontology compared to other COVID-19 related tweets.
% Toward this end, we try two simple techniques:
% \noindent \textit{(2) Embedding-based filtering:}
% This technique utilizes sentence embedding similarity to filter tweets instead of merely using keywords.
Specifically, we associate each event type with a seed repository of $5$-$10$ diverse tweets.
Query tweets are filtered out based on their sentence-level similarity (measured using the BERT sentence embedding model \cite{reimers-2019-sentence-bert}) with this event-based seed repository.
% Specifically, we curate a seed repository of $5$-$10$ diverse tweets related to each event.
% For each query tweet, we embed it using the BERT sentence embedding model \cite{reimers-2019-sentence-bert} and measure its cosine similarity with the curated tweets for each event.
% Using a similarity threshold, tweets are filtered for a particular event.
This step filters about $95\%$ tweets from our base dataset significantly reducing the annotation cost. 
% \tanmay{Can be reduced / merged with Sampling}
% \textbf{from 3\% of tweets containing at least one event to over 70\%}. 
% \alex{@Tanmay, please review this section as well}
% \noindent \textit{(1) Keyword-based filtering:}
% The core idea of this technique is curate a list of keywords specific to each event and filter out tweets containing these keywords.
% To build this list of keywords, we first curate a small list using our base event knowledge and expand this list further using synonyms from Thesaurus\footnote{\url{https://www.thesaurus.com/}}.
% We then calculate the HIT rate (percentage of tweets containing the event information) for a small sample of tweets containing these keywords.
% We filter out keywords having a low rate as they are generic and finalize the keyword list for each event.
% Finally, we filter tweets for each event using this event-specific keyword list.

% We compare both these techniques in terms of their HIT rates and tweet diversity scores in Table~\ref{tab:event-filtering-results}\tanmay{@Alex, need to make this table and write corresponding observations}.
% ...
% We use the embedding-based filtering for creating the final event-filtered dataset.

\mypar{Event-based Sampling}
\label{sec:event-based-sampling}
Random sampling of tweets would yield an uneven and COVID-biased distribution of event types for our dataset.
We instead perform a uniform sampling - wherein we over-sample tweets linked to less frequent types (e.g. \textit{prevent}) and under-sample the more frequent ones (e.g. \textit{death}).
Such an uniform sampling has proven to ensure model robustness \cite{parekh-etal-2023-geneva} - as also validated by our experiments (\S~\ref{sec:uniform-sampling}) - and in turn, would make \dataName{} generalizable to a wider range of diseases.
We sample a total of $1$,$975$ tweets which are utilized for ED annotation.

% % Utilizing our event-based filtering, we consider XX \tanmay{@Alex, fill this number} tweets suspected to adhere to the event ontology.
% Not all event types are equally mentioned on social media.
% To ensure more uniform distribution of events in our dataset, we over-sample tweets linked to less frequent types (e.g. \textit{prevent}) and under-sample the more frequent ones (e.g. \textit{death}).
% % We further select a smaller batch of tweets by over-sampling tweets linked to less frequent events (e.g. \textit{prevent}) and under-sampling the ones linked to more frequent events (e.g. \textit{death}) to have a diverse and uniformly distributed dataset adhering to our event ontology.
% This final sampling yields a total of $1$,$975$ tweets which we utilize for annotation.

% \alex{maybe call this section Tweet Selection or Document Selection}
% \begin{enumerate}
%     \item Motivation for filtering \textbf{QUESTION: should we justify why we use social media as a data source?} Yes, I think that would be helpful 
%     \tanmay{@Alex}

% We adopt Tweets from \textbf{INSERT DATASET} as the source for our data. We choose documents from Twitter over more traditional sources of data due to 
    
    % \item Initial filtering of COVID-related tweets provided by Twitter API ( We randomly selected tweets from between 15/5/2020-31/5/2020,) 
    % \tanmay{@Alex}
%     \item Keyword/trigger-based filtering. Describe the initial experiment of labeling 100-200 examples and getting keywords. Talk about keyword expansion via Thesaurus. \tanmay{@Jiarui}

% To get a set of keywords for each event, we go through two steps: The first step is building up an initial set of keywords without any knowledge from the tweet dataset. For each event, we come up with as much related keywords as we can think of. Then we obtain their synonyms via Thesaurus, adding the synonyms into the keyword set if make sense. The second step is filtering the current keyword set based on their semantic meaning in tweeter data. For each keyword, we randomly sample ten non-repeated tweets with its occurrence and manually calculate the rate of which the keyword fits the definition of its event. This rate is used as a confidence score to filter out keywords with extremely low score. In other words, if most occurrence of the keyword do not manifest the definition of its event, the keyword is removed from the set. After these two steps, we have finalized the keyword set of each event. 
    
%     \item Embedding-based similarity filtering. Describe the pipeline of how we use the initial shortlisted sentences as primary sentences. \tanmay{@Alex}
    
% To effectively construct this data set and reduce the amount of annotations needed, we utilized an embedding-based similarity filter to select tweets which were more likely to contain events. We measure the cosine-similarity of each tweet to a corpus of positive examples using a BERT-based sentence embedder \cite{reimers-2019-sentence-bert} and we only consider tweets above a certain similarity threshold. We label each tweet with a 'suspected event' based on which positive example the tweet was most similar to. We then do a random selection of tweets, biasing towards tweets with more uncommon 'suspected events' in order to construct a more balanced distribution of events in our dataset. 
%     \item Maybe some comparison (quantitative/qualitative) for keyword and embedding-based shortlisting. \tanmay{@Alex}
% \end{enumerate}

% \subsubsection{Final Tweet Selection}
% \tanmay{@Alex}

% \begin{enumerate}
%     \item Discuss dates and randomization strategies
%     \item Discuss event distribution based sampling of tweets
% \end{enumerate}

\subsection{Data Annotation}
\label{sec:data-annotation}

% After selecting candidate tweets, we annotate them based on our event ontology (\S~\ref{sec:ontology-creation}).
% In this section, we describe our process for annotating the candidate tweets based on our ontology.

% \subsubsection{Annotation Guidelines}
% \mypar{Annotation Setup}
For ED annotation, annotators are tasked with identifying whether a given tweet mentions any of the events outlined in our ontology.
If an event is indeed mentioned, annotators are required to identify the specific event trigger.
% Our annotation task requires the annotator to determine if the given tweet describes any of the events from our ontology.
% If an event exists, we require the annotator to determine the corresponding trigger.
% and label it with the corresponding event type.
Following the standard ACE dataset \cite{doddington-etal-2004-automatic}, we design our annotation guidelines and amend them through several rounds of preliminary annotations to ensure consistency amongst the annotators.
% We provide our final annotation guidelines in the Appendix 
% For our interface, we utilize Amazon Mechanical Turk.\footnote{\url{https://www.mturk.com/}}
Additional details and illustrations of the annotation guidelines and interface are provided in Appendix~\ref{sec:annotation-guidelines-interface}.
% \tanmay{Need to be linked and cleaned}.
% , but highlight some major considerations below.

% \mypar{Annotating Events:} 
% We annotate explicit as well as hypothetical and future mentions of an event (e.g. \textit{I might be infected} for the event \textit{infect}).
% We do not annotate the negation of an event or implicit and common-sense reasoning-based events (e.g. \textit{I tested negative for COVID} for the event \textit{infect}).

% \mypar{Annotating Triggers:}
% Since multiple words can indicate the presence of the event, we follow a priority order of verbs, nouns, and adjectives to reduce disagreements in annotations.
% More specifically, if the main verb is too generic or not indicative of the event, we consider the major nouns/pronouns in the sentence.
% If they are ambiguous as well, then we consider the corresponding adjectives.

% \begin{enumerate}
    % \item Describe high-level details about the annotation guidelines. Refer to the complete guidelines in the Appendix and add information there. \tanmay{@Jiarui}

% Given a tweet, each annotator has the following task: determine whether any of the event exists and choose a trigger word if an event exist. Besides the ontology, a guideline is provided to ensure that annotations across individuals are standardized instead of relying on pure intuitions.
% To summarize, the guideline stipulates situation in which an event should not exist and the predilection when choosing the trigger words. We list some bullet points below, and the complete guideline is appended in the Appendix.\\
% When deciding the existence of an event: 1) a negation of an event should not be annotated as exist to distinguish the annotation process from a keyword searching process (eg. In “I am not infected”, event “infect” does not exist); 2) the occurrence of an event must be indicated by a trigger word cannot be inferred from another event (eg. In “30 people died of COVID”, one cannot say event “infect” exist because those who died of COVID must have been infected); 3) hyperboles and rhetoric must not be identified as events …
% When choosing the trigger word: 1) looks for the main verb first before considering nouns or adjectives; 2) do not mark event arguments as triggers if there exist a synoptic trigger… \\
% Most rules in the guidelines are invoked from the ACE annotation guideline \cite{ace2005events}, and abundant examples are provided to elaborate. 

    
    % \item Discuss the MTurk Setup and how to choose multiple events and triggers. Describe examples given. Refer to image of the MTurk screen in Appendix. \tanmay{@Syed}
    % \linebreak\linebreak
    % Annotators are presented with one tweet at a time in the Amazon Mechanical Turk interface. To create an annotation, the annotator clicks on a given word twice, upon which a secondary menu with each annotation event appears. The annotator can select all event type(s) that correspond to the selected word, as well as flag the word if the annotation is ambiguous. Completed annotations appear underneath the tweet, and can be edited/removed later on. There are five tweets presented in each assignment, otherwise known as a HIT on Amazon Mechanical Turk. Once the annotator is finished with each of the tweets, the "Submit HIT" button is enabled, which allows the annotator to submit the annotations.
    
% \end{enumerate}

% \subsubsection{Annotation Setup}

% \mypar{Annotation Interface}
% We utilize Amazon Mechanical Turk\footnote{\url{https://www.mturk.com/}} as the primary interface for our annotation setup.
% To annotate, annotators can select any word and label it into one of the seven pre-defined event types.
% Event definitions and examples are provided alongside for reference.
% Each batch (also known as HIT) comprises five tweets for flexibility in annotations.
% More details and illustrations of the annotation interface are provided in the Appendix.
% \tanmay{@Syed, shift the larger set of details to the Appendix. Add link to appendix}

\mypar{Annotator Details}
To ensure high annotation quality and enforce consistency, we choose six experts instead of crowdsourced workers for our annotation.
These experts are computer science students studying NLP and are well-versed with the task of ED.
% \tanmay{@kuan-hao Do we need more details about how we choose annotators?}
They were further trained on our task through multiple loops of annotations and feedback.
% \tanmay{Can be merged with previous section}
% Along with high quality, expert annotations ensure high annotation speed with approximately 3-5 minutes per batch of five tweets.

\mypar{Inter-annotator agreement (IAA)}
We used Fleiss' Kappa \cite{fleiss1971measuring} for measuring IAA.
% \tanmay{@Kuan-Hao, how to cite?}
% To ensure high data quality,
We conduct two phases of IAA studies:
(1) \textit{Guideline Improvement:} Three annotators participated in three annotation rounds with a focus on improving the guidelines. IAA score rose from $0.44$ in the first round to $0.59$ ($70$ samples) in the final round.
(2) \textit{Agreement Improvement:} All annotators participated in three rounds of annotations. IAA score improved from $0.56$ in the first round to a strong $0.65$ ($50$ samples) in the final round.
% \begin{itemize}
%     \item \textit{Guideline Improvement:} 
%     The first phase focused on improving the guidelines by optimizing the consistency among a small group of annotators.
%     Three expert annotators participated in three rounds of annotations wherein the guidelines were modified based on the disagreement patterns among the annotators.
%     After the final round, the annotation guidelines were finalized.
%     The IAA score rose from $0.44$ in the first round to $0.59$ for $70$ tweets in the final round.
%     \item \textit{Annotator Agreement Improvement:}
%     The second phase was aimed at improving the agreement between all six annotators.
%     All six expert annotators participated in this phase in three rounds of studies.
%     The IAA score improved from $0.56$ in the first round ($50$ samples) to a decent $0.65$ in the final round ($30$ samples) of annotations.
%     \tanmay{@Jiarui, can you add the number of samples in the final round of IAA study?}
% \end{itemize}

% \begin{enumerate}
    % \item Discuss details about the annotators involved \tanmay{@Syed}
    % \linebreak\linebreak
    % Six annotators were used throughout the process, all of whom are affiliated with the UCLA ScAI Lab. Anonymous crowdsourcing of annotations (as is commonly done via Amazon Mechanical Turk) was not used in the interest of preserving quality and enforcing specific standards in regard to annotation style. Each tweet was annotated separately by at least two of the six annotators for crosschecking, and any inconsistencies or flagged tweets were resolved by a third annotator to whom both previous annotations were visible.
    
%     \item Discuss IAA studies and improvements. Enlist the final IAA score with high-level event-based statistics. \tanmay{@Jiarui}

% We adopt an iterative process involving annotation experiment and polishing event definitions. In every iteration, a group of annotators work on a set of sampled tweets, and the inter-annotator -agreement is evaluated by Fleiss Kappa, based on which an expert examines inconsistent annotation and update annotation guidelines to reduce discrepancies.

% In the incipient stage, three annotators are involved. 25 tweets are sampled based on keyword searching of events “symptom”, “infect”, and “spread”, and the initial Fleiss Kappa is 0.44. Via the first round of annotation, we discern the ambiguity among events, especially between “infect” and “spread”. This observation is further verified by a control experiment, in which the annotators annotate 20 tweets considering events “infect” and “symptom” and get a Fleiss Kappa score as high as 0.81. After modifying the guideline, annotators annotate 70 samples containing potentially all the seven events; the resulting Fleiss Kappa is 0.59.

% Overhauling the guidelines, we enter the second stage with six annotators involved, and the data sampling process takes in the consideration of all seven events. In the first round of annotation, we get an overall Fleiss Kappa of 0.56, and 3 out of six annotators agree on the occurrence of 5 out of 7 events. Yet the consistency corresponding to each event varies: “death” event has the highest FK score of 0.74 while “control” event has the lowest FK score of 0.27. Thus, in the following revision of the annotation guidelines, we further discriminant events (such as “control” vs. “prevent” and “infect” vs. “spread”) by their scale and standardize their choice of trigger words. In the last round of annotation, we get a Fleiss Kappa score 0.65. At this point the annotators are adroit at this task, so we conclude our annotation experiment and move on to the formal annotation for our dataset. 

    
% \end{enumerate}

% \subsubsection{Quality Control}
\mypar{Quality Control}
Apart from extensive IAA studies, we deploy two mechanisms to ensure the high annotation quality:
(1) \textit{Multi-Annotation:}
Each tweet is annotated by two annotators and disagreements are resolved by a third annotator.
(2) \textit{Flagging:}
Annotators can ``flag'' ambiguous annotations, which are then resolved and annotated by a third annotator through collective discussion.
% Meanwhile the flagging function is not abused: out of approximately $2000$ annotated tweets, around $370$ of them are flagged, which is less than 20\%.
% \tanmay{@Jiarui, can we have some stat about the number of flagged cases?}
Both these mechanisms along with a good IAA score ensure that the annotations have high quality.

% \begin{enumerate}
    % \item Describe the inclusion of "flag" events to handle ambiguous cases better. Also, describe how we resolve them. \tanmay{@Syed}
    % \linebreak\linebreak
    % The "flag" event was introduced to improve overall annotation quality when the word corresponding to a given event is ambiguous. This is most common when a given event corresponds to more than one word, or when no word in the tweet adequately indicates the event. Flagged tweets are resolved by a third annotator as described in the "Annotator Details" section.
    
    % \item Describe how each tweet is annotated by two experts and a third expert further if there is a disagreement between the first two experts. \tanmay{@Bonnie}
% \end{enumerate}

% \begin{table*}[ht]
%     \centering
%     \resizebox{.95\textwidth}{!}{
%     \begin{tabular}{lrrrrrrr}
%         \toprule
%         \multirow{2}{*}{\textbf{Dataset}} & \textbf{Data} & \textbf{Sentence} & \textbf{Trigger} & \textbf{Social} & \textbf{Personal} & \textbf{Social Media} \\
%         & \textbf{Source} & \textbf{Level} & \textbf{Present} & \textbf{Events} & \textbf{Events} & \textbf{Granular} \\
%         \midrule
%         \dataName{} (Ours) & Twitter & \cmark & \cmark & \cmark & \cmark & \cmark \\
%         COVIDKB \cite{zong-etal-2022-extracting} & Twitter & \cmark & \xmark & \xmark & \cmark & \cmark \\
%         CACT \cite{DBLP:journals/jbi/LybargerOTY21} & Clinical & \xmark & \xmark & \xmark & \tildemark & \cmark \\
%         ExcavatorCovid \cite{min-etal-2021-excavatorcovid} & News & \xmark & \cmark & \cmark & \cmark & \xmark \\ 
%         BioCaster \cite{DBLP:journals/bioinformatics/CollierDKGCTNDKTST08} & News & \xmark & \xmark & \cmark & \cmark & \xmark \\
%         DANIEL \cite{DBLP:journals/artmed/LejeuneBDL15} & News & \xmark & \tildemark & \xmark & \tildemark & \cmark \\
%         % Medical Reports & News & \cmark & \xmark & \xmark & \xmark \\
%         % PADI-Web \cite{VALENTIN2020105163} & News & \tildemark & \xmark & \xmark \\
%         \bottomrule
%     \end{tabular}}
%     \caption{Objective comparison of various epidemiological datasets with our dataset \dataName{}. We objectify the source of base data (Data Source), the level of annotation granularity (Sentence Level), the presence of trigger information (Trigger Present), the presence of social and personal events in ontology (Social Events and Persona Events), and the suitability of ontology for social media (Social Media Granular). \tildemark{} indicates partial presence.}
%     \label{tab:dataset-checklist}
% \end{table*}


==> sections/expt.tex <==
\section{Experimentation and Results}
% \kaiwei{combine section 5 and 6}

Previous epidemiological works majorly explore simple rule-based or simple BERT-based models (\S~\ref{sec:epi-ie-works}).
In our work, we explore recently proposed ED models for epidemiological applications for the first time.
We describe the various experimental settings (\S~\ref{sec:test-suites}), ED models (\S~\ref{sec:models}), evaluation metrics (\S~\ref{sec:eval-metrics}), and the final results (\S~\ref{sec:results}) in this section.
% We conduct a bunch of experiments in various settings to assess how current models perform in predicting pandemic-related events.
% Here, we describe the various test suites and models used for our experimentation.

\subsection{Benchmarking Test Suites}
\label{sec:test-suites}
% \tanmay{@Eric}

% \begin{enumerate}
%     \item Describe the 3-4 different data setups that we have and the use-case for each of them
% \end{enumerate}

To realistically assess the generalizability of existing ED models for epidemiological events, following \cite{parekh-etal-2023-geneva}, we focus on the following test suites:

\kuanhao{Just refactor unseen events -> transfer from existing datasets + models -> Establish it's a challenging task}

\paragraph{Unseen Events}
Since no annotated social media data is available for epidemic events, these test suites capture the ability of models to transfer to unseen event types. No training/validation data is provided in this setup.
We focus on two test suites:
\begin{enumerate}[topsep=1pt, itemsep=-2pt, leftmargin=15pt]
    \item Zero-shot (ZS): Models are only provided with the names and definitions of the events.
    \item Event Type Induction (ETI): Models are not provided with any information and discover events in a completely unsupervised manner.
    % This test suite evaluates the ability to discover unknown events without using event definitions in a completely unsupervised manner. These methods usually utilize clustering techniques on event representations. 
\end{enumerate}

\kuanhao{Now we study how much data we need to perform well on this task -> Limited Data}

\paragraph{Limited Data}
This setting focuses on the capability of models to learn and generalize from limited training data.
We focus on these two test suites:
\begin{enumerate}[topsep=1pt, itemsep=-2pt, leftmargin=15pt]
\setcounter{enumi}{2}
    \item Few-shot (FS): Models are provided access to $n$ mentions per event ($n$-shot) for training. We explore $2$-shot and $5$-shot with three splits of data in our evaluation.
    \item Low Resource (LR): Models have access to a limited $100$-$300$ event mentions for training.
    % Training data is sampled based on the ground-truth event distribution for realistic evaluation.
\end{enumerate}

\noindent We present the statistics for train-test splits of these test suites in Table~\ref{tab:data-stats-test-suites} in the Appendix (\S~\ref{sec:test-suites-statistics}).
% \tanmay{@Eric Fill the table using the data}

\subsection{Models}
\label{sec:models}

% \begin{enumerate}
%     \item Describe various models we are benchmarking organized by the data setups
% \end{enumerate}

We consider a wide range of recent ED models (implementation details in the Appendix~\ref{sec:implementation-details}) for benchmarking as organized below.
% \kuanhao{We should have the same order as the previous ones. zero-shot -> event type induction -> few-shot.}

% \paragraph{Zero-shot}
% \tanmay{@All Add your model name, citation of original paper, and one-line description of model. You can take the description (don't copy but modify) from the ZED paper.}
% For this test suite, we consider
\vspace{1pt}
\noindent \textbf{Zero-shot} models comprise
(1) \textbf{TE} \cite{lyu-etal-2021-zero}, a pre-trained model that uses event definitions to formulate ED as a textual entailment and question-answering task,
(2) \textbf{WSD} \cite{yao-etal-2021-connect} which encodes the contextualized trigger and event definitions jointly and uses a classification head atop for event detection.
% We club these models as event-definition zero-shot models.

% \paragraph{Event Type Induction} 
% We consider: 
\vspace{1pt}
\noindent \textbf{Event Type Induction} models comprise
(3) \textbf{TA{\small BS}} \cite{li-etal-2022-open}, a model that utilizes two complementary embedding spaces ("mask view" and "token view") to classify examples of new event types.
(4) \textbf{ETypeClus} \cite{shen-etal-2021-corpus}, a pipeline that extracts salient predicate-object pairs and clusters the embeddings of these pairs in a spherical latent space.
% We modify the implementations and inference methods for these models to better adapt them for ED (more details in \S~\ref{implementation-details-tabs} and \S~\ref{implementation-details-etypeclus}).
% \tanmay{@Shawn Add details and link to Appendix}

% \paragraph{Few-shot and Low Resource}
% Models considered for both these suites include:
\vspace{1pt}
\noindent \textbf{Few-shot and Low Resource} test suites include models like
(5) \textbf{DyGIE++} \cite{wadden-etal-2019-entity}, a multi-task classification-based model utilizing local and global context via span graph propagation,
(6) \textbf{BERT-QA} \cite{du-cardie-2020-event}, a classification model utilizing label semantics by formulating event detection as a question-answering task,
\kuanhao{Change BERT-QA to EE-QA}
(7) \textbf{DEGREE} \cite{hsu-etal-2022-degree}, a generation-based model prompting using natural language templates,
(8) \textbf{TagPrime} \cite{hsu-etal-2023-simple}, a sequence tagging approach that utilizes priming words to input text to convey more task-specific information.
DEGREE and TagPrime pre-trained on the ACE \cite{doddington-etal-2004-automatic} and MAVEN \cite{wang-etal-2020-maven} are also used as \textit{zero-shot pre-trained models}.
% \tanmay{Add info for MAVEN pre-trained models}

% \paragraph{Other Baselines}
% We consider a couple of other baseline models:
\vspace{1pt}
\noindent \textbf{Other baselines} that we consider include
(9) \textbf{Keyword} \cite{DBLP:journals/artmed/LejeuneBDL15}, a popular epidemiological model, that predicts an event if any of the event-specific curated keywords are present in the sentence,
(10) \textbf{GPT-3} \cite{brown2020language}, a large-language model (LLM) baseline using GPT-3.5-turbo as the base model with seven in-context examples.
% \tanmay{Should we run zero-shot GPT experiments?}

\subsection{Evaluation Metrics}
\label{sec:eval-metrics}
% \tanmay{@Tanmay}

% Describe the general evaluation metrics for the task.

Following previous works \cite{ahn-2006-stages}, we report the F1-score for the two tasks of Trigger identification (\textbf{Tri-I}) and trigger classification (\textbf{Tri-C}) respectively.
For few-shot and low-resource suites, we report the average scores over three model runs.
% For event-type induction, we use ... \tanmay{@Shawn add this part once you finalize evaluation}


==> sections/intro-ie-kh.tex <==
\section{Introduction}

Early epidemic warnings and effective control measures are among the most important tools for policymakers to be prepared against the threat of any epidemic \cite{DBLP:journals/bioinformatics/CollierDKGCTNDKTST08}.
World Health Organization (WHO) reports suggest that $65\%$ of the first reports about infectious diseases and outbreaks originate from informal sources and the internet \cite{heymann2001hot}.
Social media becomes an important information source here, as it's more timely than other alternatives like news and public health \cite{lamb-etal-2013-separating}, more publicly accessible than clinical notes \cite{DBLP:journals/jbi/LybargerOTY21}, and possesses a huge volume of content.\footnote{A daily average of 20 million tweets were posted about COVID-19 from May 15 -- May 31, 2020.}
In our work, we explore the social application of information extraction towards building an automated system to efficiently extract epidemic events from social media to provide better epidemic preparedness.
% This underscores the need for an automated system to monitor and efficiently extract epidemic events from social media to provide better epidemic preparedness, which we explore in our work

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{images/mpox-total-trend.pdf}
    \caption{Number of reported Monkeypox cases and the number of extracted events from our trained BERT-QA model from May 11 to Nov 11, 2022. Indicated arrows show how our system can potentially provide early epidemic warnings almost 4-8 weeks before the WHO declared Monkeypox as a pandemic.}
    \label{fig:mpox-total-trend}
\end{figure}
% \alex{what does the figure show? add a opinionated sentence in the caption. For example, our system successfully warns/detects the spread of an unseen epidemic before xxx. - Yufei. (targeted at the sentence 'Arrows indicate the early epidemic warning by our system'.)}

The process of identifying and categorizing significant events based on a pre-defined ontology is a well-established task in NLP, known as \textit{Event Detection} (ED) \cite{sundheim-1992-overview, doddington-etal-2004-automatic}.
However, standard ED datasets mostly focus on general-purpose events for news or Wikipedia domains, and can't be transferred to the epidemic domain (\S~\ref{sec:prev-methods-results}).
% \kuanhao{Add one sentence saying that there cannot be generalized to epidemic domain and refer to the later section.}
% Although ED has been explored for epidemiological tasks, 
Furthermore, 
most prior epidemiological ED ontologies restrict themselves only to certain diseases or are too fine-grained and specific in nature; while the corresponding datasets majorly focus on news or clinical domains (\S~\ref{sec:related-works}).
% \kuanhao{Do we discuss this point later or in the appendix? If yes, we can refer to the corresponding section.}
Thus, existing ED ontologies and datasets are not sufficient and models trained on them cannot be readily utilized for extracting events from social media for emerging epidemics.
% Event Detection (ED) is a well-established task \cite{sundheim-1992-overview, doddington-etal-2004-automatic} that aims at identifying and categorizing significant events based on a pre-defined ontology.
% Recent progress has vastly improved the task performance by improving datasets \cite{} and creating robust models \cite{}.
% However, the application of this task for social impact and real-life applications has been under-explored.
% While recent advancements have notably improved task performance through large datasets \cite{wang-etal-2020-maven, parekh-etal-2023-geneva} and robust modeling \cite{hsu-etal-2022-degree, wang-etal-2023-code4struct}, the practical application of this task for societal impact and real-world use cases remains largely unexplored.
% In our work, we examine a socially impactful application of ED for detecting events in social media with the goal of providing better epidemic preparedness.

% Small paragraph motivating the need for such a system.

% Epidemic early warnings and effective control measures are among the most important tools for policymakers to be prepared against the threat of any epidemic \cite{DBLP:journals/bioinformatics/CollierDKGCTNDKTST08}.
% World Health Organization (WHO) reports suggest that $65\%$ of the first reports on events about infectious diseases originate from informal sources and the internet \cite{heymann2001hot}.
% Here, social media becomes an important information source, as it's more timely than other alternatives like news and public health \cite{lamb-etal-2013-separating}, more publicly accessible than clinical notes \cite{DBLP:journals/jbi/LybargerOTY21}, and possesses a huge volume of content.\footnote{A daily average of 20 million tweets were posted about COVID-19 from May 15 -- May 31, 2020.}
% In our work, we explore the applicability of ED for monitoring and extracting epidemic events from social media with a larger social impact of providing better epidemic preparedness.
% \kuanhao{Actually I like the previous version better. Emphasizing pandemic first and saying that current ED datasets are not enough.}
% This underscores the need for an automated system to monitor and efficiently extract epidemic events from social media to provide better epidemic preparedness.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\columnwidth]{images/cover.pdf}
%     \caption{Illustration of how Event Detection can be used to detect various epidemic-related events and ensure better preparedness.}
%     \label{fig:cover-image}
% \end{figure}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\columnwidth]{images/cover-narrow.pdf}
%     \caption{Illustration of how Event Detection can be used to detect various epidemic events and promote better epidemic preparedness.}
%     \label{fig:cover-image}
% \end{figure}

% Standard ED datasets mostly focus on general-purpose events for news or Wikipedia domains.
% Although ED has been explored for epidemiological tasks, most prior epidemiological ontologies restrict themselves only to certain diseases or are too fine-grained and specific in nature.
% Moreover, the corresponding datasets also majorly focus on news or clinical domains.
% Thus, existing ED ontologies and datasets are not sufficient and models trained on them cannot be readily utilized for extracting events from social media for any new epidemic.

% The usage of ED for epidemiological tracking and prediction is widely prevalent~\cite{mutuvi-etal-2020-dataset,sahnoun-lejeune-2021-multilingual}.
% However, most prior epidemiological ontologies are specific only to certain diseases \cite{DBLP:conf/icbo/He0OWLHHBLDAXHY20}, are too fine-grained \cite{min-etal-2021-excavatorcovid} or focus only on certain event types \cite{DBLP:journals/jbi/LybargerOTY21}.
% Moreover, the corresponding datasets also majorly focus on news \cite{DBLP:journals/bioinformatics/CollierDKGCTNDKTST08, DBLP:conf/tsd/DuEKNTY11} or clinical domains \cite{DBLP:journals/jbi/LybargerOTY21}.
% How these can't be used or will not generalize well.
% Thus, existing epidemiological ontologies and datasets are not sufficient and models trained on them cannot be readily utilized for extracting events from social media for any new epidemic.
% \kaiwei{Reduce extent of epidemiological comparison}

To this end, we construct our own epidemic ED ontology and dataset for social media.
Our ontology comprises seven event types - \textit{infect}, \textit{spread}, \textit{symptom}, \textit{prevent}, \textit{cure}, \textit{control}, \textit{death} - chosen based on their relevance for epidemic preparedness, frequency of mentions in social media, and their applicability to various diseases.
Our ontology and event definitions are derived from clinical sources \cite{DBLP:journals/bioinformatics/CollierDKGCTNDKTST08,DBLP:journals/biomedsem/BabcockBCS21} and its sufficiency and coverage are validated by public health experts and quantitative analyses.
% \tanmay{Based on our final analysis, add ontology coverage summary here.}
For our dataset, we choose Twitter as the social media platform and focus on the recent COVID-19 pandemic.
Since our task requires domain expertise, we hire six expert annotators
% (students well-versed in NLP) instead of crowdsourced workers
to ensure high annotation quality for our dataset.
Using our curated ontology and expert annotation, we create our epidemic preparedness dataset \textbf{\dataName{}} (\textbf{S}ocial \textbf{P}latform based \textbf{E}pidemic \textbf{E}vent \textbf{D}etection) comprising $1$,$975$ tweets and $2$,$217$ event mentions.
\dataName{} provides good coverage of events characteristic of any disease and is granular for social media; thus, serves as a valuable ED benchmark for epidemic preparedness from social media.

% To this end, we construct our own epidemic ED ontology and dataset for social media.
% Our ontology comprises seven event types - \textit{infect}, \textit{spread}, \textit{symptom}, \textit{prevent}, \textit{cure}, \textit{control}, \textit{death} - chosen based on their relevance for epidemic preparedness and frequency of mentions in social media.
% Our ontology and event definitions are derived from clinical sources \cite{DBLP:journals/bioinformatics/CollierDKGCTNDKTST08,DBLP:journals/biomedsem/BabcockBCS21} and validated by public health experts.
% For our dataset, we choose Twitter as the social media platform and focus on the recent COVID-19 pandemic.
% Since our task requires domain expertise, we hire six expert annotators (students well-versed in NLP) instead of crowdsourced workers to ensure high annotation quality for our dataset.
% Using our curated ontology and expert annotation, we create our epidemic preparedness dataset \textbf{\dataName{}} (\textbf{S}ocial \textbf{P}latform based \textbf{E}pidemic \textbf{E}vent \textbf{D}etection) comprising $1$,$975$ tweets and $2$,$217$ event mentions.
% \dataName{} provides good coverage of events characteristic of any disease and is granular for social media; thus, serves as a valuable ED benchmark for epidemic preparedness from social media.

% Based on their relevance for epidemic preparedness and frequency of mentions in social media, we curate seven event types - \textit{infect}, \textit{spread}, \textit{symptom}, \textit{prevent}, \textit{cure}, \textit{control}, \textit{death} - for our ontology.

We benchmark various existing models including four zero-shot models \cite{shen-etal-2021-corpus, lyu-etal-2021-zero} and two supervised models \cite{hsu-etal-2022-degree} pre-trained on existing ED datasets of ACE \cite{doddington-etal-2004-automatic} and MAVEN \cite{wang-etal-2020-maven} on our \dataName{} benchmark.
% \tanmay{do we need to add citations here?} \violet{yes, we'd better do.}
Experiments reveal that none of the existing models perform well on our dataset mainly owing to the domain-shift and noise in social media as well as unseen epidemic-based event types.
Furthermore, training on limited in-domain \dataName{} data provides significant gains compared to the existing models, highlighting the importance of domain-specific training.
Overall, these results reveal how \dataName{} is a challenging ED dataset.

% Despite great advances in model generalizability for ED,
% most prior works use keyword-based \cite{DBLP:journals/artmed/LejeuneBDL15}, rule-based \cite{DBLP:journals/bioinformatics/CollierDKGCTNDKTST08, lamb-etal-2013-separating}, or simple BERT-based \cite{DBLP:journals/bioinformatics/MengOPSPFGZKBC22} models.
% In our work, \violet{I suggest removing the above passage -- no need to criticize prior models as this is not your focus.}
% We benchmark a diverse set of $10$ ED models including many recently proposed ones \cite{du-cardie-2020-event, hsu-etal-2023-simple} on our dataset by designing four different test suites.
% % \kaiwei{Just say we benchmark 9 ED models and how these models generalize to this domain/task. Replace 1st and 2nd line or push to related work. Also avoid saying "SOTA" models, replace to "new/recently proposed".}
% These suites realistically assess the models' ability to generalize to epidemic events using zero to limited in-domain training data.
% Experiments reveal that zero-shot models (no in-domain training data) perform very poorly owing to noisy social media text and unseen event types. 
% \kuanhao{Add line about poor transfer from existing datasets.}
% % \wei{do we have citations?}
% On the other hand, a small amount of in-domain training data ($30$-$300$ event mentions) provides consistently stronger model performance.
% One more line based on model performance comparison with older methods (mention first to show such a comparison) ...

% Finally, we study the generalizability of our COVID-only dataset \dataName{} for any emerging epidemics.
Tying back to our original motivation of epidemic preparedness, we evaluate the utility and generalizability of our COVID-only dataset \dataName{} to detect events for any emerging epidemics.
% \violet{I would frame this differently. Instead of saying study the generalizability, I'll tie this back to our original motivation, which is to use ED for epidemic preparation, we'll say we use this dataset to test our hypothesis and see whether our dataset can provide early warning for other epidemics.}
More specifically, we evaluate models trained only on \dataName{} to detect events for three unforeseen epidemics of \textit{Monkeypox}, \textit{Zika}, and \textit{Dengue}.
% without training on any target epidemic data.
Experiments reveal that \dataName{}-trained models can successfully detect events for all these epidemics while providing improvements of $29\%$ F1 over zero-shot models and $10\%$ F1 over supervised models trained on small samples of target epidemic data. 
Furthermore, by comparing the trends of our extracted events with the actual reported cases, we show that our model can provide early preparedness warnings for the Monkeypox epidemic (Figure~\ref{fig:mpox-total-trend}).
These results underscore the strong generalizability and applicability of our dataset \dataName{} for general epidemic preparedness.

% To ensure robust epidemic preparedness, models need to be generalizable to detect event mentions for any emerging epidemic.
% We demonstrate the generalization of our ED framework by evaluating it for detecting events for an unseen potential epidemic of \textit{Monkeypox}.
% We show that all ED models trained on our in-domain COVID-19 dataset can successfully detect events for Monkeypox and provide significant improvements up to $29\%$ F1 over the models using no in-domain data.
% Furthermore, by comparing the trends of our extracted events with the actual reported cases, we show that our model can provide early preparedness warnings for the Monkeypox epidemic (Figure~\ref{fig:mpox-total-trend}).

Overall, we make the following contributions:
(1) We create an ED ontology and dataset \dataName{} tailored for predicting epidemic events charactersitc of any disease from social media,
% (2) We benchmark $10$ ED models on four test suites using our dataset highlighting the significance of our in-domain training data, \kuanhao{This contribution is not clear for me. Maybe saying that our experimental results show that existing datasets cannot be transferred well to our dataset and therefore emphasize the importance of our dataset?}
(2) We show that existing zero-shot models and datasets cannot transfer well to our dataset, highlighting the significance of our dataset,
(3) We validate the generalizability of our framework by demonstrating how \dataName{}-trained ED models using only COVID-tweets can successfully detect events and provide early warnings for three unforeseen epidemics.
% In conclusion, our work lays solid foundations for utilizing social media to ensure better epidemic preparedness.
% \tanmay{To add line for early warnings}
% \kaiwei{Finetuning on in-domain data can lead to better generalizability.}

% \tanmay{Should we shift related works to section 2?}

==> sections/intro-ie.tex <==
\section{Introduction}

Event Detection (ED) is a well-established task \cite{sundheim-1992-overview, doddington-etal-2004-automatic} that aims at identifying and categorizing significant events based on a pre-defined ontology.
% Recent progress has vastly improved the task performance by improving datasets \cite{} and creating robust models \cite{}.
% However, the application of this task for social impact and real-life applications has been under-explored.
While recent advancements have notably improved task performance through large datasets \cite{wang-etal-2020-maven, parekh-etal-2023-geneva} and robust modeling \cite{hsu-etal-2022-degree, wang-etal-2023-code4struct}, the practical application of this task for societal impact and real-world use cases remains largely unexplored.
% In our work, we examine a socially impactful application of ED for detecting events in social media with the goal of providing better epidemic preparedness.

% Small paragraph motivating the need for such a system.

Epidemic early warnings and effective control measures are among the most important tools for policymakers to be prepared against the threat of any epidemic \cite{DBLP:journals/bioinformatics/CollierDKGCTNDKTST08}.
World Health Organization (WHO) reports suggest that $65\%$ of the first reports on events about infectious diseases originate from informal sources and the internet \cite{heymann2001hot}.
Here, social media becomes an important information source, as it's more timely than other alternatives like news and public health \cite{lamb-etal-2013-separating}, more publicly accessible than clinical notes \cite{DBLP:journals/jbi/LybargerOTY21}, and possesses a huge volume of content.\footnote{A daily average of 20 million tweets were posted about COVID-19 from May 15 -- May 31, 2020.}
In our work, we explore the applicability of ED for monitoring and extracting epidemic events from social media with a larger social impact of providing better epidemic preparedness.
\kuanhao{Actually I like the previous version better. Emphasizing pandemic first and saying that current ED datasets are not enough.}
% This underscores the need for an automated system to monitor and efficiently extract epidemic events from social media to provide better epidemic preparedness.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\columnwidth]{images/cover.pdf}
%     \caption{Illustration of how Event Detection can be used to detect various epidemic-related events and ensure better preparedness.}
%     \label{fig:cover-image}
% \end{figure}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\columnwidth]{images/cover-narrow.pdf}
%     \caption{Illustration of how Event Detection can be used to detect various epidemic events and promote better epidemic preparedness.}
%     \label{fig:cover-image}
% \end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{images/mpox-total-trend.pdf}
    \caption{Number of reported Monkeypox cases and the number of extracted events from our trained BERT-QA model from May 11 to Nov 11, 2022. Arrows indicate the early epidemic warnings by our system.}
    \label{fig:mpox-total-trend}
\end{figure}

Standard ED datasets mostly focus on general-purpose events for news or Wikipedia domains.
Although ED has been explored for epidemiological tasks, most prior epidemiological ontologies restrict themselves only to certain diseases or are too fine-grained and specific in nature.
Moreover, the corresponding datasets also majorly focus on news or clinical domains.
Thus, existing ED ontologies and datasets are not sufficient and models trained on them cannot be readily utilized for extracting events from social media for any new epidemic.

% The usage of ED for epidemiological tracking and prediction is widely prevalent~\cite{mutuvi-etal-2020-dataset,sahnoun-lejeune-2021-multilingual}.
% However, most prior epidemiological ontologies are specific only to certain diseases \cite{DBLP:conf/icbo/He0OWLHHBLDAXHY20}, are too fine-grained \cite{min-etal-2021-excavatorcovid} or focus only on certain event types \cite{DBLP:journals/jbi/LybargerOTY21}.
% Moreover, the corresponding datasets also majorly focus on news \cite{DBLP:journals/bioinformatics/CollierDKGCTNDKTST08, DBLP:conf/tsd/DuEKNTY11} or clinical domains \cite{DBLP:journals/jbi/LybargerOTY21}.
% How these can't be used or will not generalize well.
% Thus, existing epidemiological ontologies and datasets are not sufficient and models trained on them cannot be readily utilized for extracting events from social media for any new epidemic.
% \kaiwei{Reduce extent of epidemiological comparison}

To this end, we construct our own epidemic ED ontology and dataset for social media.
Our ontology comprises seven event types - \textit{infect}, \textit{spread}, \textit{symptom}, \textit{prevent}, \textit{cure}, \textit{control}, \textit{death} - chosen based on their relevance for epidemic preparedness, frequency of mentions in social media, and their applicability to various diseases.
Our ontology and event definitions are derived from clinical sources \cite{DBLP:journals/bioinformatics/CollierDKGCTNDKTST08,DBLP:journals/biomedsem/BabcockBCS21} and its sufficiency and coverage are validated by public health experts and quantitative analyses.
% \tanmay{Based on our final analysis, add ontology coverage summary here.}
For our dataset, we choose Twitter as the social media platform and focus on the recent COVID-19 pandemic.
Since our task requires domain expertise, we hire six expert annotators
% (students well-versed in NLP) instead of crowdsourced workers
to ensure high annotation quality for our dataset.
Using our curated ontology and expert annotation, we create our epidemic preparedness dataset \textbf{\dataName{}} (\textbf{S}ocial \textbf{P}latform based \textbf{E}pidemic \textbf{E}vent \textbf{D}etection) comprising $1$,$975$ tweets and $2$,$217$ event mentions.
\dataName{} provides good coverage of events characteristic of any disease and is granular for social media; thus, serves as a valuable ED benchmark for epidemic preparedness from social media.

% To this end, we construct our own epidemic ED ontology and dataset for social media.
% Our ontology comprises seven event types - \textit{infect}, \textit{spread}, \textit{symptom}, \textit{prevent}, \textit{cure}, \textit{control}, \textit{death} - chosen based on their relevance for epidemic preparedness and frequency of mentions in social media.
% Our ontology and event definitions are derived from clinical sources \cite{DBLP:journals/bioinformatics/CollierDKGCTNDKTST08,DBLP:journals/biomedsem/BabcockBCS21} and validated by public health experts.
% For our dataset, we choose Twitter as the social media platform and focus on the recent COVID-19 pandemic.
% Since our task requires domain expertise, we hire six expert annotators (students well-versed in NLP) instead of crowdsourced workers to ensure high annotation quality for our dataset.
% Using our curated ontology and expert annotation, we create our epidemic preparedness dataset \textbf{\dataName{}} (\textbf{S}ocial \textbf{P}latform based \textbf{E}pidemic \textbf{E}vent \textbf{D}etection) comprising $1$,$975$ tweets and $2$,$217$ event mentions.
% \dataName{} provides good coverage of events characteristic of any disease and is granular for social media; thus, serves as a valuable ED benchmark for epidemic preparedness from social media.

% Based on their relevance for epidemic preparedness and frequency of mentions in social media, we curate seven event types - \textit{infect}, \textit{spread}, \textit{symptom}, \textit{prevent}, \textit{cure}, \textit{control}, \textit{death} - for our ontology.


% Despite great advances in model generalizability for ED,
% most prior works use keyword-based \cite{DBLP:journals/artmed/LejeuneBDL15}, rule-based \cite{DBLP:journals/bioinformatics/CollierDKGCTNDKTST08, lamb-etal-2013-separating}, or simple BERT-based \cite{DBLP:journals/bioinformatics/MengOPSPFGZKBC22} models.
% In our work, \violet{I suggest removing the above passage -- no need to criticize prior models as this is not your focus.}
We benchmark a diverse set of $10$ ED models including many recently proposed ones \cite{du-cardie-2020-event, hsu-etal-2023-simple} on our dataset by designing four different test suites.
% \kaiwei{Just say we benchmark 9 ED models and how these models generalize to this domain/task. Replace 1st and 2nd line or push to related work. Also avoid saying "SOTA" models, replace to "new/recently proposed".}
These suites realistically assess the models' ability to generalize to epidemic events using zero to limited in-domain training data.
Experiments reveal that zero-shot models (no in-domain training data) perform very poorly owing to noisy social media text and unseen event types. 
\kuanhao{Add line about poor transfer from existing datasets.}
% \wei{do we have citations?}
On the other hand, a small amount of in-domain training data ($30$-$300$ event mentions) provides consistently stronger model performance.
% One more line based on model performance comparison with older methods (mention first to show such a comparison) ...

Finally, we study the generalizability of our COVID-only dataset \dataName{} for any emerging epidemics. \violet{I would frame this differently. Instead of saying study the generalizability, I'll tie this back to our original motivation, which is to use ED for epidemic preparation, we'll say we use this dataset to test our hypothesis and see whether our dataset can provide early warning for other epidemics.}
More specifically, we evaluate models trained only on \dataName{} to detect events for three unforeseen epidemics of \textit{Monkeypox}, \textit{Zika}, and \textit{Dengue} without training on any target epidemic data.
Experiments reveal that \dataName{}-trained models can successfully detect events for all these epidemics while providing improvements of $29\%$ F1 over zero-shot models and $10\%$ F1 over supervised models trained on small samples of target epidemic data. 
Furthermore, by comparing the trends of our extracted events with the actual reported cases, we show that our model can provide early preparedness warnings for the Monkeypox epidemic (Figure~\ref{fig:mpox-total-trend}).
These results highlight the strong generalizability and applicability of our dataset \dataName{} for any emerging epidemic.

% To ensure robust epidemic preparedness, models need to be generalizable to detect event mentions for any emerging epidemic.
% We demonstrate the generalization of our ED framework by evaluating it for detecting events for an unseen potential epidemic of \textit{Monkeypox}.
% We show that all ED models trained on our in-domain COVID-19 dataset can successfully detect events for Monkeypox and provide significant improvements up to $29\%$ F1 over the models using no in-domain data.
% Furthermore, by comparing the trends of our extracted events with the actual reported cases, we show that our model can provide early preparedness warnings for the Monkeypox epidemic (Figure~\ref{fig:mpox-total-trend}).

Overall, we make the following contributions:
(1) We create an ED ontology and dataset \dataName{} tailored for predicting epidemic events from social media,
(2) We benchmark $10$ ED models on four test suites using our dataset highlighting the significance of our in-domain training data, \kuanhao{This contribution is not clear for me. Maybe saying that our experimental results show that existing datasets cannot be transferred well to our dataset and therefore emphasize the importance of our dataset?}
(3) We validate the generalizability of our framework by demonstrating how \dataName{}-trained ED models containing only COVID-related tweets can successfully detect events and provide early warnings for three unforeseen epidemics.
% In conclusion, our work lays solid foundations for utilizing social media to ensure better epidemic preparedness.
% \tanmay{To add line for early warnings}
% \kaiwei{Finetuning on in-domain data can lead to better generalizability.}

% \tanmay{Should we shift related works to section 2?}

==> sections/intro-new.tex <==
\section{Introduction}

Early warnings and effective control measures are among the most important tools for policymakers to be prepared against the threat of any epidemic \cite{DBLP:journals/bioinformatics/CollierDKGCTNDKTST08}.
World Health Organization (WHO) reports suggest that $65\%$ of the first reports on events about infectious diseases and outbreaks originate from informal sources and the internet \cite{heymann2001hot}.
Social media becomes an important information source here, as it's more timely than other alternatives like news and public health \cite{lamb-etal-2013-separating}, more publicly accessible than clinical notes \cite{DBLP:journals/jbi/LybargerOTY21}, and possesses a huge volume of content.\footnote{A daily average of 20 million tweets were posted about COVID-19 from May 15 -- May 31, 2020.}
% In recent times, the prevalence of such event mentions has grown significantly on social media platforms \cite{lamb-etal-2013-separating}, with a daily average of 20 million 
% \tanmay{@Alex, double-check please?} 
% tweets posted on Twitter discussing the recent COVID-19 pandemic.\footnote{Average recorded between May 15 -- May 31, 2020}
This underscores the need for an automated system to monitor and efficiently extract epidemic events from social media to provide better epidemic preparedness.
% \violet{I think it's too early to bring up this generalizability consideration. should probably move it to later.} More importantly, for optimal epidemic preparedness, we require these models and corresponding datasets and ontologies to be generalizable to detect event mentions for any emerging epidemic.
% Therefore \kuanhao{This is a bit weird to me. It feels like we are going to propose a new method that is more generalizable as the solution. I would choose to emphasize no good epidemic dataset a bit more so that's why we need new ontology and dataset.}, the generalizability of automated frameworks to detect event mentions for potential new epidemics serves as the cornerstone for improving epidemic preparedness.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\columnwidth]{images/cover.pdf}
%     \caption{Illustration of how Event Detection can be used to detect various epidemic-related events and ensure better preparedness.}
%     \label{fig:cover-image}
% \end{figure}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\columnwidth]{images/cover-narrow.pdf}
%     \caption{Illustration of how Event Detection can be used to detect various epidemic events and promote better epidemic preparedness.}
%     \label{fig:cover-image}
% \end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{images/mpox-total-trend.pdf}
    \caption{Number of reported Monkeypox cases and the number of extracted events from our trained BERT-QA model from May 11 to Nov 11, 2022. Arrows indicate the early epidemic warnings by our system.}
    \label{fig:mpox-total-trend}
\end{figure}

The process of identifying and categorizing significant events based on a pre-defined ontology is a well-established task in NLP, known as \textit{Event Detection} (ED).
% One of the relevant tasks in NLP for this application is Event Detection (ED), which identifies and categorizes essential events based on a pre-defined ontology \cite{luan-etal-2019-general,lin-etal-2020-joint,wang-etal-2020-maven}.
% \tanmay{@kuan-hao, add citation}
The usage of ED for epidemiological tracking and prediction is widely prevalent~\cite{mutuvi-etal-2020-dataset,sahnoun-lejeune-2021-multilingual}.
% It is prevalent to use ED for epidemiological tracking and prediction~\cite{mutuvi-etal-2020-dataset,sahnoun-lejeune-2021-multilingual}. 
% \tanmay{add two early citations here}
% Line about issues with prior datasets/ontologies.
However, most prior epidemiological ontologies are specific only to certain diseases \cite{DBLP:conf/icbo/He0OWLHHBLDAXHY20}, are too fine-grained \cite{min-etal-2021-excavatorcovid} or focus only on certain event types \cite{DBLP:journals/jbi/LybargerOTY21}.
% \violet{unclear what's the difference of ``restricted to specific diseases'' and ``extract only specific events''}
Moreover, the corresponding datasets also majorly focus on news \cite{DBLP:journals/bioinformatics/CollierDKGCTNDKTST08, DBLP:conf/tsd/DuEKNTY11} or clinical domains \cite{DBLP:journals/jbi/LybargerOTY21}.
% How these can't be used or will not generalize well.
Thus, existing epidemiological ontologies and datasets are not sufficient and models trained on them cannot be readily utilized for extracting events from social media for any new epidemic.
\kaiwei{Reduce extent of epidemiological comparison}

To this end, we construct our own epidemic ED ontology and dataset for social media.
Our ontology comprises seven event types - \textit{infect}, \textit{spread}, \textit{symptom}, \textit{prevent}, \textit{cure}, \textit{control}, \textit{death} - chosen based on their relevance for epidemic preparedness, frequency of mentions in social media, and their applicability to various diseases.
Our ontology and event definitions are derived from clinical sources \cite{DBLP:journals/bioinformatics/CollierDKGCTNDKTST08,DBLP:journals/biomedsem/BabcockBCS21} and validated by public health experts.
\tanmay{Based on our final analysis, add ontology coverage summary here.}
For our dataset, we choose Twitter as the social media platform and focus on the recent COVID-19 pandemic.
Since our task requires domain expertise, we hire six expert annotators
% (students well-versed in NLP) instead of crowdsourced workers
to ensure high annotation quality for our dataset.
Using our curated ontology and expert annotation, we create our epidemic preparedness dataset \textbf{\dataName{}} (\textbf{S}ocial \textbf{P}latform based \textbf{E}pidemic \textbf{E}vent \textbf{D}etection) comprising $1$,$975$ tweets and $2$,$217$ event mentions.
\dataName{} provides good coverage of events characteristic of any disease and is granular for social media; thus, serves as a valuable ED benchmark for epidemic preparedness from social media.

% To this end, we construct our own epidemic ED ontology and dataset for social media.
% Our ontology comprises seven event types - \textit{infect}, \textit{spread}, \textit{symptom}, \textit{prevent}, \textit{cure}, \textit{control}, \textit{death} - chosen based on their relevance for epidemic preparedness and frequency of mentions in social media.
% Our ontology and event definitions are derived from clinical sources \cite{DBLP:journals/bioinformatics/CollierDKGCTNDKTST08,DBLP:journals/biomedsem/BabcockBCS21} and validated by public health experts.
% For our dataset, we choose Twitter as the social media platform and focus on the recent COVID-19 pandemic.
% Since our task requires domain expertise, we hire six expert annotators (students well-versed in NLP) instead of crowdsourced workers to ensure high annotation quality for our dataset.
% Using our curated ontology and expert annotation, we create our epidemic preparedness dataset \textbf{\dataName{}} (\textbf{S}ocial \textbf{P}latform based \textbf{E}pidemic \textbf{E}vent \textbf{D}etection) comprising $1$,$975$ tweets and $2$,$217$ event mentions.
% \dataName{} provides good coverage of events characteristic of any disease and is granular for social media; thus, serves as a valuable ED benchmark for epidemic preparedness from social media.

% Based on their relevance for epidemic preparedness and frequency of mentions in social media, we curate seven event types - \textit{infect}, \textit{spread}, \textit{symptom}, \textit{prevent}, \textit{cure}, \textit{control}, \textit{death} - for our ontology.


% Despite great advances in model generalizability for ED,
% most prior works use keyword-based \cite{DBLP:journals/artmed/LejeuneBDL15}, rule-based \cite{DBLP:journals/bioinformatics/CollierDKGCTNDKTST08, lamb-etal-2013-separating}, or simple BERT-based \cite{DBLP:journals/bioinformatics/MengOPSPFGZKBC22} models.
% In our work, \violet{I suggest removing the above passage -- no need to criticize prior models as this is not your focus.}
We benchmark a diverse set of $10$ ED models including many recently proposed ones \cite{du-cardie-2020-event, hsu-etal-2023-simple} on our dataset by designing four different test suites.
% \kaiwei{Just say we benchmark 9 ED models and how these models generalize to this domain/task. Replace 1st and 2nd line or push to related work. Also avoid saying "SOTA" models, replace to "new/recently proposed".}
These suites realistically assess the models' ability to generalize to epidemic events using zero to limited in-domain training data.
Experiments reveal that zero-shot models (no in-domain training data) perform very poorly owing to noisy social media text and unseen event types. 
% \wei{do we have citations?}
On the other hand, a small amount of in-domain training data ($30$-$300$ event mentions) provides consistently stronger model performance.
% One more line based on model performance comparison with older methods (mention first to show such a comparison) ...

Lastly, we study the generalizability of our COVID-only dataset \dataName{} for any emerging epidemics.
More specifically, we evaluate models trained only on \dataName{} to detect events for three unforeseen epidemics of \textit{Monkeypox}, \textit{Zika}, and \textit{Dengue} without training on any target epidemic data.
Experiments reveal that \dataName{}-trained models can successfully detect events for all these epidemics while providing improvements of $29\%$ F1 over zero-shot models and $10\%$ F1 over supervised models trained on small samples of target epidemic data. 
Furthermore, by comparing the trends of our extracted events with the actual reported cases, we show that our model can provide early preparedness warnings for the Monkeypox epidemic (Figure~\ref{fig:mpox-total-trend}).
These results highlight the strong generalizability and applicability of our dataset \dataName{} for any emerging epidemic.

% To ensure robust epidemic preparedness, models need to be generalizable to detect event mentions for any emerging epidemic.
% We demonstrate the generalization of our ED framework by evaluating it for detecting events for an unseen potential epidemic of \textit{Monkeypox}.
% We show that all ED models trained on our in-domain COVID-19 dataset can successfully detect events for Monkeypox and provide significant improvements up to $29\%$ F1 over the models using no in-domain data.
% Furthermore, by comparing the trends of our extracted events with the actual reported cases, we show that our model can provide early preparedness warnings for the Monkeypox epidemic (Figure~\ref{fig:mpox-total-trend}).

Overall, we make the following contributions:
(1) We create an ED ontology and dataset \dataName{} tailored for predicting epidemic events from social media,
(2) We benchmark $10$ ED models on four test suites using our dataset highlighting the significance of our in-domain training data,
(3) We validate the generalizability of our framework by demonstrating how \dataName{}-trained ED models (without using any target epidemic data) can successfully detect events and provide early warnings for three unforeseen epidemics.
% In conclusion, our work lays solid foundations for utilizing social media to ensure better epidemic preparedness.
% \tanmay{To add line for early warnings}
% \kaiwei{Finetuning on in-domain data can lead to better generalizability.}

% \tanmay{Should we shift related works to section 2?}

==> sections/intro.tex <==
\section{Introduction}

% Main thing

% Importance of early warnings and control measures for policy makers in handling any pandemic.
% 65\% of early reports on infections/control comes through informal sources on the internet - back in 2001.
% This is more prevalent in social media in today's era and more so for the recent COVID-19 pandemic.
% Loads of posts on social media daily, impossible to manually trace what people talk about.
% Need a strong automated tracking system to monitor and find relevant information about early signals and control measures that people are using.

Early warnings and effective control measures are among the most important tools for policymakers to be prepared against the threat of any epidemic \cite{DBLP:journals/bioinformatics/CollierDKGCTNDKTST08}.
World Health Organization (WHO) reports suggest that $65\%$ of the first reports on events about infectious diseases and outbreaks originate from informal sources and the internet \cite{heymann2001hot}.
In recent times, the prevalence of such event mentions has grown significantly on social media platforms \cite{lamb-etal-2013-separating}, with an average of XX 
\tanmay{@Alex, can you help fill this number based on average for our data?} 
tweets per day recorded on Twitter discussing the recent COVID-19 pandemic.\footnote{Need to add more details about time}
% These social media posts can be utilized to extract epidemic-relevant events, which 
% but given their sheer volume, it is practically impossible to do so manually \hb{it seems obvious why extracting epidemic relevant info cannot be done manually. write something else about extracting epidemic relevant info which is more useful.}. 
This underscores the imperative need for an automated framework capable of monitoring and efficiently extracting epidemic events from social media.
Previous works \cite{DBLP:journals/bioinformatics/CollierDKGCTNDKTST08, DBLP:journals/artmed/LejeuneBDL15} relying on keyword matching and simple NLP techniques are not robust and fail to detect emerging epidemics and diseases.
Therefore \kuanhao{This is a bit weird to me. It feels like we are going to propose a new method that is more generalizable as the solution. I would choose to emphasize no good epidemic dataset a bit more so that's why we need new ontology and dataset.}, the generalizability of automated frameworks to detect event mentions for potential new epidemics serves as the cornerstone for improving epidemic preparedness.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{images/cover-image.png}
    \caption{Illustration of how Event Detection can be used to detect various epidemic-related events and ensure better preparedness.}
    \label{fig:cover-image}
\end{figure}


% Introduce the task of event detection.
% Discuss about some progress in event detection and how it can successfully detect important events.
% Previous works have used this technique too for other applications (find) and for COVID information monitoring too.
% Following some previous works, we use event detection for monitoring this information.
% But our application focuses more on general pandemic-related information tracking to provide early signals and control measures.
One of the relevant tasks in NLP for this application is Event Detection (ED), which entails identifying and categorizing essential events based on a pre-defined ontology.
\tanmay{@kuan-hao, add citation}
% Notably, over the years, there has been significant progress in constructing ED datasets \cite{song-etal-2015-light, wang-etal-2020-maven, zhan2023glen} and developing stronger ED model \cite{} \tanmay{Need to add 3 major papers here}.
ED models have been successfully deployed in various NLP applications such as question-answering \cite{DBLP:conf/sigir/YangCWK03, han-etal-2021-ester}, information retrieval \cite{DBLP:conf/aiia/BasileCSS14a}, knowledge graphs \cite{DBLP:conf/www/ZhangLPSL20} as well as information tracking for COVID \cite{min-etal-2021-excavatorcovid, zong-etal-2022-extracting}.
In our work, we utilize ED for identifying epidemic events from social media generalizable for any emerging epidemic, as shown in Figure~\ref{fig:cover-image}.
\tanmay{TThis is a reference pic, will be updated}
\kuanhao{I feel like we should talk about the advantages of ED, like it can extract concepts and identify relationships between entities, rather than saying its applications.}
% \hb{what is general epidemic}.
% We believe this \hb{rather than we believe say that our system will provide..} generalization will provide better future epidemic preparedness as described in Figure~\ref{fig:cover-image}.
% emphasize need for generalizability
% \hb{since the submission has to be completely blind, maybe you wouldn't want to mention UCLA in the figure 1. }
% \hb{the figure is a bit unclear to me specifically the green and yellow box. Who Where and Symptom for Infection are event arg roles right? Detecting these in a tweet should be referred to as Event Extraction which is more than Event Detection. Please correct me if I am understanding it incorrectly.}

Toward this end, 
% \hb{i am not sure that the problem statement is super clear and hence towards this end is not making a lot of sense.},
we construct our own event ontology and a corresponding benchmarking dataset \dataName{} for epidemic events.
% \hb{cut `in our work'}
% \hb{i am not sure if you have established a need for epidemic specific event ontology -- need to talk about existing ontologies and how they are ill-characteristics for pandemics.}.
Most previous epidemiological ED ontologies are restricted to surface-level or specific events only and corresponding datasets majorly focus on news or clinical domains \cite{DBLP:journals/artmed/LejeuneBDL15, mutuvi-etal-2020-dataset, zong-etal-2022-extracting} 
Consequentially, they can't be readily used for extracting epidemic events from social media.
% \hb{last 2 lines should have come earlier and then say something like "To this end, we ...}.
\tanmay{Should we change the flow to put the last two lines above?}
\kuanhao{We need to explain the reasons more clearly. For example, if there is a new disease their anthologies would fail...}

Inspired by these epidemiological event ontologies, we construct our ontology comprising seven event types - \textit{infect}, \textit{spread}, \textit{symptom}, \textit{prevent}, \textit{cure}, \textit{control}, \textit{death} - that are characteristic for any epidemic. 
\kuanhao{Emphasize that we follow the real medical or clinical definitions.}
% \hb{may need a better word instead of generalizable -- i have seen generalizable in the context of models and rarely in the context of dataset. Maybe you need something like: "our event ontology covers a broad spectrum of event types that are characteristic for any epidemic."}
For our dataset, we choose Twitter as the social media platform and focus on the recent COVID-19 pandemic.
% \hb{talk about how you accomplish this.}
\hb{i would like to see some discussion on prior works (if any) who have tried to do something like this, and how you position yourself in comparison to them.}
% Since there are millions of tweets daily \hb{millions of tweets in total or just COVID-19 tweets?},
% most of which are irrelevant to our ontology \hb{this is too obvious},
Given \kuanhao{This sentence is redundant for me. I have a different opinion from Hritk's comment. I think we don't need to spend too much on the details about processing tweets. Instead, we should talk more about the advantage of our dataset and the difference from previous ones.} the sheer volume of daily tweets,
we build a pipeline using sentence-embedding similarities to automatically filter epidemic-relevant tweets.
% \hb{how to you filter -- 1line on the approach}
We hire six expert annotators to annotate these filtered tweets and create our epidemic preparedness benchmarking dataset \dataName{} comprising $1$,$975$ tweets and $2$,$217$ event mentions.
\kuanhao{Need a transition here. Mention why our dataset is a good one for benchmark.}
% \hb{need to mention something like: "We provide more details for the data construction process in Section.."} 

% To develop a strong ED framework for this application, we need a relevant event ontology along with a corresponding dataset for training and evaluation of the models.
% Most previous ontologies for pandemic-related ED are restricted to surface-level or specific events and corresponding datasets majorly focus on news or clinical domains \cite{DBLP:journals/artmed/LejeuneBDL15, mutuvi-etal-2020-dataset, zong-etal-2022-extracting}.
% Consequentially, they can't be readily used for ED for pandemic prediction and control from social media.

% Towards this end, we construct our own event ontology and dataset in our work.
% First, we study various epidemiological event ontologies and construct our ontology comprising seven events relevant to the detection and control of infectious diseases.
% For our dataset, we choose Twitter as the social media platform and focus on tweets related to the recent COVID-19 pandemic.
% Since there are millions of tweets daily, most of which are irrelevant to our pandemic ontology, we build a filtering pipeline to automatically select tweets most relevant to our ontology.
% We hire six expert annotators to annotate these filtered tweets based on our curated ontology and create our benchmarking dataset \dataName{} comprising $1$,$975$ tweets and $2$,$217$ event mentions.

% After building this dataset, we benchmark existing models on four realistic benchmarking test suites categorized in unseen and limited data settings.
% We observe that models struggle in the unseen setting, but are much better when trained on small amounts of data.
% This shows how model transfer for ED in social media on new events is far more difficult.
% But also that using small amount of data for training can strongly boost model performance.

We benchmark a diverse set of $XX$ \tanmay{to be updated} ED models \tanmay{We have many models, citations needed? Also, should we specify more details about them?} on our dataset by designing four test suites.
% \hb{good to cite the ED models here}
% \hb{there is a disconnect with the last paragraph. it is unclear as to why any ED model can be evaluated on your dataset since current ED models would not understand your epidemic ontology}
% including one based on large language models (LLM) \hb{why do you need to mention this explicitly}.
% for predicting our epidemic preparedness events.
These suites realistically assess the models' ability to generalize to epidemic events using zero to limited in-domain training data.
% \hb{how did you get from one dataset PIPP to 4 benchmarking test suites?}
Experimental results reveal that zero-shot models (no in-domain training data) perform very poorly owing to noisy social media text and new event types.
On the other hand, a small amount of in-domain training data ($30$-$300$ event mentions) leads to a consistently stronger ED performance.
% \hb{i would love to know more about the models you tried.}
% \hb{in the context of 1975 tweets, 300 instances seems a lot so cannot say a small amount of in-domain training data}
One more line based on model performance ...

Finally, to demonstrate the transferability and generalization of our ED ontology and modeling, we evaluate our framework for detecting events for an unseen \tanmay{is there a need to justify how it is unseen or not in our training data already?} potential epidemic of \textit{Monkeypox} (Mpox).
% \hb{i am a bit conflicted here -- generalizability is often referred to the models instead of the data. If your model performs well on Mpox then is the model able to generalize or is the dataset able to generalize. i think the idea is there but need to use the right terms.}.
We observe that all ED models
% \hb{does it happen for all the models or any specific set of models?} 
trained on our curated COVID-19 \dataName{} dataset can successfully detect events for Monkeypox and provide significant improvements upto $30$ F1 points over the zero-shot baseline models.
One more line based on final analysis ...
\kuanhao{How about training with monkeypox and testing on our dataset? After reading this paragraph I would first suspect that the two datasets have the same domain knowledge.}

Overall, in our work, we make the following contributions:
% \hb{should be inside enumerate as separate points.}
(1) We create an event ontology
% \hb{sounds strange Event Detection Event Ontology}
and benchmarking dataset \dataName{} tailored for predicting events promoting epidemic preparedness from social media,
(2) We benchmark $XX$ \tanmay{To be filled} ED models on four test suites using our dataset highlighting the challenges of this task,
(3) We demonstrate the generalizability of our framework by utilizing ED models trained on our COVID-19 dataset for successfully detecting events for an unseen epidemic of Monkeypox.
% \hb{i am on the fence due to my incomplete understanding of the work -- but what measures does the training data takes to make sure that there is no monkeypox epidemic information in it. I think such minor details can enrich the introduction more.
\hb{i think it is missing how or whether clinicians were involved in any stage of the dataset creation. if there are any related works that support your choice of event types, then it would be very good to cite them. i feel there are very few related papers cited in the introduction. are their any Bio-Event detection models, BioMedLLMs that are open-sourced? if there are not, then you should add as a contribution that you will publicly release the first ever biomed-event detection model.}

\tanmay{Should we shift related works to section 2?}

==> sections/limited-data-results.tex <==
\subsection{Training with Limited \dataName{} Data}
\label{sec:limited-data-results}

% \kuanhao{Indicate what our conclusion will be at the start to highlight it better}

To improve performance, we train ED models using limited in-domain \dataName{} training data.
We consider two training paradigms:
\textbf{Few-shot (FS)} models are trained on $n$ mentions per event ($n$-shot). We use $n=2$ and $5$.
\textbf{Low Resource (LR)} models are trained on limited $100$-$300$ event mentions
(more details in Table~\ref{tab:data-stats-test-suites} in \S~\ref{sec:test-suites-statistics}).

We train the following ED models:
(1) DyGIE++ \cite{wadden-etal-2019-entity},
(2) BERT-QA \cite{du-cardie-2020-event},
(3) DEGREE \cite{hsu-etal-2022-degree},
(4) TagPrime \cite{hsu-etal-2023-simple}.
Other baselines also include
(5) Keyword \cite{DBLP:journals/artmed/LejeuneBDL15}, an epidemiological model utilizing event-specific \textit{curated} keywords, and
(6) GPT-3 \cite{brown2020language}, a large-language model (LLM) baseline using GPT-3.5-turbo.
% (5) \textbf{Keyword} \cite{DBLP:journals/artmed/LejeuneBDL15}, an epidemiological model utilizing event-specific \textit{curated} keywords for classification,
% (6) \textbf{GPT-3} \cite{brown2020language}, a large-language model (LLM) baseline using GPT-3.5-turbo as the base model with seven \textit{in-context} examples.

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{images/limited-data-results.pdf}
    \caption{Model performances on the Few-Shot (FS)  and Low Resource (LR) test suites in terms of Tri-C F1 scores. Here, LR-XX represents low resource with XX training event mentions and FS-Y represents few-shot with Y training mentions per event.}
    \label{fig:results-ld-plot}
\end{figure}

\paragraph{Results}

% We follow the same evaluation setup described in \S~\ref{sec:prev-work-eval}.
Figure~\ref{fig:results-ld-plot} presents the model performances.
% in terms of Tri-C scores. 
% for the few-shot and low-resource settings.
% Figure~\ref{fig:results-ld-plot} presents the model performances on the few-shot and low-resource test suites.
% Majorly, we observe how increasing in-domain training data yields improvements in performance consistently for all models.
% With higher amounts of training data, TagPrime performs the best, while in the few-shot setting, DyGIE++ and BERT-QA perform better. 
Majorly, we observe how training on in-domain data can yield gains upto $50$ F1 points over the zero-shot and data-transfer methods.
GPT-3 and Keyword baselines are also easily outperformed by models trained on just $30$ event mentions.
% $28$ F1 points compared to strong GPT-3 and Keyword baselines.
% Furthermore, these gains are highly consistent for the different ED models.
Overall, we note the \textbf{significance of \dataName{} as small amounts of in-domain training data can provide significant gains} in model performance.
% compared to the existing zero-shot and data-transfer models.

% \kuanhao{Combine section 4 and 5 - make it short. Name it why is SPEED important? Some message in this and next section tying to why is SPEED important.}

==> sections/monkeypox.tex <==
\section{Generalization for New Epidemics}
\label{sec:new-pandemic}

% \begin{table}[t]
%     \centering
%     \begin{tabular}{lcc|cc}
%         \toprule
%         \multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{c|}{\textbf{F1}} & \multicolumn{2}{c}{\textbf{Recall (Tri-C)}} \\
%         & \textbf{Tri-I} & \textbf{Tri-C} & \textbf{mpox} & \textbf{non}\\
%         \midrule
%         \multicolumn{5}{c}{\textsc{Baseline Models}} \\
%         \midrule
%         TE & 16.70 & 12.11 & 8.65 & 3.67 \\
%         WSD & 22.04 & 4.35 & 97.25 & 81.08 \\
%         GPT-3 & $42.23$ & $35.33$ & $43.25$ & $46.79$ \\
%         \midrule
%         \multicolumn{5}{c}{\textsc{\dataName{} Fine-tuned Models}} \\
%         \midrule
%         BERT-QA & $\textbf{67.38}$ & $\textbf{64.17}$ & $\textbf{61.94}$ & $\textbf{55.96}$ \\
%         DEGREE & $62.95$ & $61.45$ & $53.98$ & $55.05$ \\
%         TagPrime & $64.71$ & $61.92$ & $57.44$ & $51.38$ \\
%         DyGIE++ & $62.76$ & $59.82$ & $52.6$ & $47.71$ \\
%         \bottomrule
%     \end{tabular}
%     \caption{Benchmarking results for event detection on a new epidemic of \textit{Monkeypox}. The second and third columns report \textbf{F1} scores for Tri-I and Tri-C tasks, respectively. The fourth and fifth columns report the \textbf{Recall} for Tri-C split by Monkeypox (\textbf{mpox}) and Non-monkeypox (\textbf{non}) events.}
%     \label{tab:monkeypox-results}
% \end{table}

Since \dataName{} focuses only on the COVID-19 pandemic, its transferability for detecting events for new epidemics remains unknown.
To effectively evaluate this generalization, we test if ED models trained on our in-domain COVID dataset can detect events for an unseen epidemic.
We consider the outbreak of \textit{Monkeypox} (\textit{Mpox}) as the unseen epidemic.
There is no data contamination since the Monkeypox outbreak started in May 2022 while \dataName{} comprises tweets dated back to May 2020.

\paragraph{Test Data Creation}
We create a test dataset utilizing the MonkeyPox2022Tweets dataset \cite{DBLP:data/10/Thakur22b}, which is a large repository of $500,000$ Monkeypox tweets.
We sample a small number of tweets and annotate them using our expert annotators.
% for creating event annotations for these tweets.
Our final evaluation dataset comprises $286$ tweets and $398$ event mentions (statistics in \S~\ref{sec:mpox-data-statistics}).
Since there were other ongoing outbreaks at the same time, not all event mentions are linked to Monkeypox.
Overall, we recorded $289$ event mentions for Monkeypox while the remaining $109$ are related to COVID, polio, and other diseases.

\paragraph{Experimental Setup}
We split \dataName{} into 80-20 training and validation splits and train various ED models.
We also benchmark the best ED models requiring no training data for comparison.
We use the overall F1 score and the recall specifically on the \textit{mpox} event mentions as the evaluation metrics.
% We also split the model performances in terms of recall for \textit{mpox} event mentions for detailed analysis.
% \tanmay{Few-shot mpox baseline?}
% \kaiwei{With/without in-domain training}
% \kaiwei{Can remove non-mpox numbers. Doesn't add value.}

% \begin{table}[t]
%     \centering
%     \begin{tabular}{lcc|cc}
%         \toprule
%         \multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{c|}{\textbf{Overall-F1}} & \multicolumn{2}{c}{\textbf{mpox-Recall}} \\
%         & \textbf{Tri-I} & \textbf{Tri-C} & \textbf{Tri-I} & \textbf{Tri-C}\\
%         \midrule
%         \multicolumn{5}{c}{\small \textsc{No In-domain Data}} \\
%         \hline
%         TE & $16.70$ & $12.11$ & $8.65$ & $3.67$ \\
%         WSD & $22.04$ & $4.35$ & $\textbf{97.25}$ & $\textbf{97.25}$ \\
%         ETypeClus & $18.31$ & $6.78$ & $80.97$ & $38.03$ \\
%         Keyword & $36.4$ & $25.09$ & $26.64$ & $19.38$ \\
%         GPT-3$^*$ & $42.23$ & $35.33$ & $53.63$ & $43.25$ \\
%         \hline
%         \multicolumn{5}{c}{\small \textsc{Fine-tuned on In-domain Data}} \\
%         \hline
%         BERT-QA & $\textbf{67.38}$ & $\textbf{64.17}$ & $65.05$ & $61.94$ \\
%         DEGREE & $62.95$ & $61.45$ & $55.02$ & $53.98$ \\
%         TagPrime & $64.71$ & $61.92$ & $59.52$ & $57.44$ \\
%         DyGIE++ & $62.76$ & $59.82$ & $54.33$ & $52.6$ \\
%         \bottomrule
%     \end{tabular}
%     \caption{Benchmarking results for event detection on a new epidemic of \textit{Monkeypox}. We report overall \textbf{F1} scores (2nd, 3rd columns), and the specific \textbf{Recall} for Monkeypox (\textbf{mpox}) event mentions. *GPT-3 uses $7$ in-domain examples as in-context examples.}
%     \label{tab:monkeypox-results}
% \end{table}
% \violet{it seems for recall, you should highlight the WSD row}

\begin{table}[t]
    \centering
    \begin{tabular}{lcc|cc}
        \toprule
        \multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{c|}{\textbf{Monkeypox}} & \multicolumn{2}{c}{\textbf{Zika/Dengue}} \\
        & \textbf{Tri-I} & \textbf{Tri-C} & \textbf{Tri-I} & \textbf{Tri-C}\\
        \midrule
        \multicolumn{5}{c}{\small \textsc{No In-domain Data}} \\
        \hline
        TE & $16.70$ & $12.11$ &  \\
        WSD & $22.04$ & $4.35$ &  \\
        ETypeClus & $18.31$ & $6.78$ & $13.99$ & $5.33$ \\
        Keyword & $36.40$ & $25.09$ &  \\
        GPT-3$^*$ & $42.23$ & $35.33$ &  \\
        \hline
        \multicolumn{5}{c}{\small \textsc{Domain Transfer from In-domain COVID Data}} \\
        \hline
        BERT-QA & $\textbf{67.38}$ & $\textbf{64.17}$ & $69.29$ & $62.47$ \\
        DEGREE & $62.95$ & $61.45$ & $67.85$ & $63.72$ \\
        TagPrime & $64.71$ & $61.92$ & $65.10$ & $60.64$ \\
        DyGIE++ & $62.76$ & $59.82$ & $\textbf{69.36}$ & $\textbf{64.16}$ \\
        \hline
        \multicolumn{5}{c}{\small \textsc{Fine-tuned on Actual Epidemic Data}} \\
        \hline
        BERT-QA & $59.8$ & $54.08$ \\
        DEGREE & $59.58$ & $54.12$ \\
        TagPrime & $55.57$ & $49.65$ \\
        DyGIE++ & $55.83$ & $50.31$ \\
        \bottomrule
    \end{tabular}
    \caption{Benchmarking results for event detection on a new epidemic of \textit{Monkeypox}. We report overall \textbf{F1} scores (2nd, 3rd columns), and the specific \textbf{Recall} for Monkeypox (\textbf{mpox}) event mentions. *GPT-3 uses $7$ in-domain examples as in-context examples.}
    \label{tab:monkeypox-results}
\end{table}
\tanmay{Need to fix how it's written/formatted}

\paragraph{Results}
We present our results in Table~\ref{tab:monkeypox-results}.
Without any in-domain data, the model performance is sub-par, with GPT-3 performing the best.
Although WSD/ETypeClus have a high recall, their precisions are low.
On the other hand, all models fine-tuned on our in-domain training data consistently provide stronger performances.
Our best model - BERT-QA - achieves an improvement of almost $29$ F1 points over the GPT baseline.
% In conclusion, training ED models on our in-domain \dataName{} dataset can provide good generalization for detecting events for any new epidemic.
% First, we observe how the baseline models perform poorly, indicating how zero-shot ED models and even LLMs would not be as successful in detecting Monkeypox events.
% Next, we observe that models trained on \dataName{} dataset perform quite well and even super close to the few-shot upper bound.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\columnwidth]{images/mpox-total-trend.pdf}
%     \caption{Number of reported Monkeypox cases and the number of extracted events from our trained BERT-QA model from May 11 to Nov 11, 2022. Arrows indicate the early warnings by our system.}
%     \label{fig:mpox-trends}
% \end{figure}

\paragraph{Can we Provide Early Epidemic Warnings?}

The final evaluation of our work is its utility for providing early signals for \textit{Monkeypox} epidemic before the outbreak actually happened.
We report the number of epidemic events extracted by our best-trained model BERT-QA along with the actual number of Mpox cases reported in the US\footnote{As reported by CDC at \url{https://www.cdc.gov/poxvirus/mpox/response/2022/mpx-trends.html}} from May 11 to Nov 11, 2022, in Figure~\ref{fig:mpox-total-trend}.
As shown by the arrows in the figure, our model could potentially provide two sets of early warnings around May 23 and June 29 before the outbreak reached its peak around July 30.
In fact, all our trained ED models are capable of providing these early signals (with varying intensities) as shown in Figure~\ref{fig:mpox-4-ED-models}.
We provide further analysis in the Appendix~\ref{sec:mpox-trends-appendix}.

In conclusion, through our generalization analysis, we demonstrate how all ED models trained on our in-domain COVID dataset can consistently detect events as well as provide early warnings for an unseen epidemic.
Thus, our dataset \dataName{} lays a strong foundational cornerstone for utilizing social media for promoting better epidemic preparedness.
% prove the utility of our work for promoting better epidemic preparedness.

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{images/MPOX_four_ED_models.pdf}
    \caption{Number of reported Monkeypox cases and the number of extracted events from four trained models from May 11 to Nov 11, 2022.}
    \label{fig:mpox-4-ED-models}
\end{figure}


==> sections/prev-work-results.tex <==
\subsection{Transfer Existing Methods} 
\label{sec:prev-methods-results}

% Since existing ED datasets and models are based on general-purpose event ontologies and news/wikipedia domains, they may not transfer well to our social-media-based epidemic detection task.
In order to verify if existing methods can directly transfer to \dataName{} (without further training), we benchmark the following families of ED models:
% For this experimentation, we assume no access to any annotated social media data for epidemic events.
% and utilize zero-shot models and models trained on existing datasets like ACE \cite{doddington-etal-2004-automatic} and MAVEN \cite{wang-etal-2020-maven} to transfer to \dataName{}.
% We majorly consider the following two families of models:

% \noindent \textbf{Zero-shot} models do not train on any supervised data and solely utilize the event definitions.
% For this, we consider
% (1) \textbf{TE} \cite{lyu-etal-2021-zero}, a pre-trained model that formulates ED as a textual entailment and question-answering task,
% (2) \textbf{WSD} \cite{yao-etal-2021-connect} which classifies based on the joint encoding of the contextualized trigger and event definitions,
% % jointly and uses a classification head atop for event detection.
% (3) \textbf{TA{\small BS}} \cite{li-etal-2022-open}, that utilizes two complementary trigger embedding spaces for classification,
% (4) \textbf{ETypeClus} \cite{shen-etal-2021-corpus}, that extracts salient predicate-object pairs and clusters their embeddings in a spherical latent space.

\noindent \textbf{Zero-shot} models do not train on any supervised data and solely utilize the event definitions.
For this, we consider
(1) TE \cite{lyu-etal-2021-zero},
(2) WSD \cite{yao-etal-2021-connect},
(3) TA{\small BS} \cite{li-etal-2022-open},
(4) ETypeClus \cite{shen-etal-2021-corpus}.

\noindent \textbf{Data transfer} models are supervised models pre-trained on standard ED datasets ACE \cite{doddington-etal-2004-automatic} and MAVEN \cite{wang-etal-2020-maven} and transfer to \dataName{} without further fine-tuning.
% (without training on any \dataName{} data).
For this, we consider
(5) DEGREE \cite{hsu-etal-2022-degree},
(6) TagPrime \cite{hsu-etal-2023-simple}.

\begin{table}[t]
    \centering
    \small
    \begin{tabular}{lcc}
        \toprule
        \textbf{Model} & \textbf{Tri-I} & \textbf{Tri-C} \\
        \midrule
        % Random & & \\
        % Majority & & \\ 
        % \hline
        \multicolumn{3}{c}{\small \textsc{Data-Transfer}} \\ 
        \midrule
        ACE - TagPrime & $0$ & $0$ \\
        % BERT-QA & $24.64$ & $0$ \\
        ACE - DEGREE & $1.82$ & $1.71$ \\
        MAVEN - TagPrime & $\textbf{27.65}$ & $0$ \\
        MAVEN - DEGREE & $26.72$ & $0$ \\
        \midrule
        \multicolumn{3}{c}{\small\textsc{Zero-Shot}} \\ 
        \midrule
        TE & $9.64$ & $5.54$ \\
        WSD & $17.68$ & $3.65$ \\
        % \midrule
        % \multicolumn{3}{c}{\small \textsc{Event Type Induction}} \\ 
        % \midrule
        TA{\small BS} & $3.70$ & $1.61$ \\
        ETypeClus & $17.56$ & $\textbf{7.66}$\\
        \bottomrule
    \end{tabular}
    \caption{Benchmarking zero-shot and data-transfer models on \dataName{} in terms of Tri-I and Tri-C F1 scores.}
    \label{tab:results-zs}
\end{table}

\paragraph{Results}
\label{sec:prev-work-eval}

% We evaluate the above models on the $1,683$ tweets from the \dataName{} dataset.
% Following previous works \cite{ahn-2006-stages}, we report the F1-score for the two tasks of Trigger identification (\textbf{Tri-I}) and trigger classification (\textbf{Tri-C}) respectively.
We present the benchmarking results in Table~\ref{tab:results-zs}.
We observe that models pre-trained on ACE and MAVEN absolutely fail to transfer to SPEED with negligible Tri-C scores.
% We observe that models pre-trained on the news dataset ACE absolutely fail, while Wikipedia dataset MAVEN pre-training improves Tri-I scores, but negligible Tri-C scores.
% to detect any events and this can be partly attributed to the domain shift between news and social media.
% \tanmay{Add comment based on MAVEN experiments}
% \tanmay{Link hows ED from different domains doesn't help here}
Zero-shot models perform only slightly better, with the best performance by ETypeClus.
Overall, \textbf{all existing zero-shot and data-transfer models fail to detect epidemic events}, mainly owing to the domain shift of social media and unseen epidemic events.
\textbf{This renders \dataName{} as a challenging ED dataset.}
% Overall, owing to the domain shift of social media data and the finer granularity of epidemic events, we observe that \textbf{all families of zero-shot models fail to detect epidemic events}.

==> sections/results.tex <==
% \subsection{Results}
% % \tanmay{@All}

% % \begin{enumerate}
% %     \item Organize results based on different data setups and show the results
% %     \item Have some analysis for the best model performances
% %     \item Real-life scenario: Monkeypox / new COVID data analysis \tanmay{@Tanmay, Shawn}
% % \end{enumerate}

% We present the results of our experimentation on the various test suites for the \dataName{} dataset in this section.
% Furthermore, we provide also some analyses to ... 

\begin{table}[t]
    \centering
    \small
    \begin{tabular}{lcc}
        \toprule
        \textbf{Model} & \textbf{Tri-I} & \textbf{Tri-C} \\
        \midrule
        % Random & & \\
        % Majority & & \\ 
        % \hline
        \multicolumn{3}{c}{\small \textsc{Pre-Trained Models}} \\ 
        \midrule
        ACE - TagPrime & $0$ & $0$ \\
        % BERT-QA & $24.64$ & $0$ \\
        ACE - DEGREE & $1.82$ & $1.71$ \\
        MAVEN - TagPrime & $\textbf{27.65}$ & $0$ \\
        MAVEN - DEGREE & $26.72$ & $0$ \\
        \midrule
        \multicolumn{3}{c}{\small\textsc{Zero-Shot}} \\ 
        \midrule
        TE & $9.64$ & $5.54$ \\
        WSD & $17.68$ & $3.65$ \\
        \midrule
        \multicolumn{3}{c}{\small \textsc{Event Type Induction}} \\ 
        \midrule
        TA{\small BS} & $3.70$ & $1.61$ \\
        ETypeClus & $17.56$ & $\textbf{7.66}$\\
        \bottomrule
    \end{tabular}
    \caption{Model performances on the Unseen Events test suites in terms of Tri-I and Tri-C F1 scores.}
    \label{tab:results-zs}
\end{table}

\subsection{Results}
\label{sec:results}

We organize our results and observations based on the two major evaluation setups:

% \begin{table*}[ht]
%     \centering
%     \begin{tabular}{l|cc|cc|cc|cc|cc}
%         \toprule
%         \multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{c|}{\textbf{FS-2}} & \multicolumn{2}{c|}{\textbf{FS-5}} & \multicolumn{2}{c|}{\textbf{LR-100}} & \multicolumn{2}{c|}{\textbf{LR-200}} & \multicolumn{2}{c}{\textbf{LR-300}} \\
%         & \textbf{Tri-I} & \textbf{Tri-C} & \textbf{Tri-I} & \textbf{Tri-C} & \textbf{Tri-I} & \textbf{Tri-C} & \textbf{Tri-I} & \textbf{Tri-C} & \textbf{Tri-I} & \textbf{Tri-C} \\
%         \midrule
%         BERT-QA & $30.21$ & $25.51$ & $45.83$ & $40.88$ & $53.90$ & $47.28$ & $61.15$ & $55.08$ & $63.17$ & $56.99$ \\
%         DEGREE & $22.32$ & $16.88$ & $41.94$ & $38.52$ & $53.14$ & $48.39$ & $58.90$ & $54.61$ & $61.34$ & $56.78$ \\
%         TagPrime & $3.32$ & $2.20$ & $31.68$ & $29.04$ & $\textbf{57.43}$ & $\textbf{52.24}$ & $61.27$ & $\textbf{57.08}$ & $\textbf{64.15}$ & $\textbf{59.24}$ \\
%         DyGIE++ & $17.81$ & $14.59$ & $\textbf{47.89}$ & $\textbf{41.45}$ & $55.33$ & $48.68$ & $\textbf{61.73}$ & $56.04$ & $63.84$ & $57.65$ \\
%         GPT-3 & $\textbf{39.36}^*$ & $\textbf{30.76}^*$ & - & - & - & - & - & - & - & - \\
%         \bottomrule
%     \end{tabular}
%     \caption{Model performances on the Few-Shot (FS)  and Low Resource (LR) test suites in terms of Tri-I and Tri-C F1 scores. Here, LR-XX represents low resource with XX training event mentions and FS-YY represents few-shot with YY training mentions per event. *experiments run under FS-1 setting and text-matching based evaluation.}
%     \label{tab:results-ld}
% \end{table*}

% \begin{table}[t]
%     \centering
%     \begin{tabular}{lrr}
%         \toprule
%         \textbf{Model} & \textbf{Tri-I} & \textbf{Tri-C} \\
%         \midrule
%         & & \\
%         \bottomrule
%     \end{tabular}
%     \caption{Model performances on the Event Type Induction (ETI) test suite in terms of Tri-I and Tri-C F1 scores.}
%     \label{tab:results-eti}
% \end{table}

\paragraph{Unseen Events}
We present the results for zero-shot model performance and event type induction in Table~\ref{tab:results-zs}.
We observe that models pre-trained on the news dataset ACE absolutely fail, while Wikipedia dataset MAVEN pre-training helps to improve Tri-I scores, but still has poor Tri-C scores.
% to detect any events and this can be partly attributed to the domain shift between news and social media.
% \tanmay{Add comment based on MAVEN experiments}
% \tanmay{Link hows ED from different domains doesn't help here}
The zero-shot models using event definitions perform slightly better, while the best performance is provided by ETypeClus which is an unsupervised ETI-based model.
Overall, owing to the domain shift of social media data and the finer granularity of epidemic events, we observe that \textbf{all families of zero-shot models fail to detect epidemic events}.
% \kuanhao{update numbers for tagprime, degree. Remove bert-qa}
% This can be majorly attributed to the domain shift of social media data and the finer granularity of epidemic events.

% \tanmay{Will be interesting to show that transfer to news/wiki domain is much easier for models than transfer to social media domain.}

\paragraph{Limited Data}
Figure~\ref{fig:results-ld-plot} presents the model performances on the few-shot and low-resource test suites.
First, we observe that increasing in-domain training data yields improvements in performance consistently for all models.
With higher amounts of training data, TagPrime performs the best, while in the few-shot setting, DyGIE++ and BERT-QA perform better. 
We also note that GPT-3 and Keyword baselines are easily outperformed by models trained with just $30$ event mentions.
Overall, we note that \textbf{small amounts of in-domain training data can provide strong performances for epidemiological ED from social media}.
% \tanmay{Add line about real-data evaluation and link to appendix}

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{images/limited-data-results.pdf}
    \caption{Model performances on the Few-Shot (FS)  and Low Resource (LR) test suites in terms of Tri-C F1 scores. Here, LR-XX represents low resource with XX training event mentions and FS-Y represents few-shot with Y training mentions per event.}
    \label{fig:results-ld-plot}
\end{figure}


